Tailed Low-Rank Matrix Factorization for Similarity Matrix Completion

Similarity matrix serves as a fundamental tool at the core of numerous downstream machine-learning tasks. However, missing data is inevitable and often results in an inaccurate similarity matrix. To address this issue, Similarity Matrix Completion (SMC) methods have been proposed, but they suffer from high computation complexity due to the Singular Value Decomposition (SVD) operation. To reduce the computation complexity, Matrix Factorization (MF) techniques are more explicit and frequently applied to provide a low-rank solution, but the exact low-rank optimal solution can not be guaranteed since it suffers from a non-convex structure. In this paper, we introduce a novel SMC framework that offers a more reliable and efficient solution. Specifically, beyond simply utilizing the unique Positive Semi-definiteness (PSD) property to guide the completion process, our approach further complements a carefully designed rank-minimization regularizer, aiming to achieve an optimal and low-rank solution. Based on the key insights that the underlying PSD property and Low-Rank property improve the SMC performance, we present two novel, scalable, and effective algorithms, SMCNN and SMCNmF, which investigate the PSD property to guide the estimation process and incorporate nonconvex low-rank regularizer to ensure the low-rank solution. Theoretical analysis ensures better estimation performance and convergence speed. Empirical results on real-world datasets demonstrate the superiority and efficiency of our proposed methods compared to various baseline methods.

==> Figure/Converge/ConvergeTable.tex <==
\begin{figure*}[!htb]
    \centering   
    \hspace{-5cm}
      \subfigure[(a) ImageNet]{
   \includegraphics[width = 0.18\columnwidth, trim=15 0 30 10, clip]{Figure/Converge/I07.eps}}
      \subfigure[(b) MNIST]{
   \includegraphics[width = 0.18\columnwidth, trim=15 0 30 10, clip]{Figure/Converge/M07.eps}}
      \subfigure[(c) PROTEIN]{
   \includegraphics[width = 0.18\columnwidth, trim=15 0 30 10, clip]{Figure/Converge/P07.eps}}
      \subfigure[(d) CIFAR]{ 
   \includegraphics[width = 0.18\columnwidth, trim=15 0 30 10, clip]{Figure/Converge/C07.eps}}
    \subfigure[(e) GoogleNews]{ 
   \includegraphics[width = 0.18\columnwidth, trim=15 0 30 10, clip]{Figure/Converge/G07.eps}}
    \hspace{-5cm}
   \caption{Tolerance on various datasets, with $m=1,000$ search candidates and $n=200$ query items, where missing ratio $\rho=0.7$, rank $r=100$,$\lambda = 0.001$, $\gamma=0.001$, iterations $T=10,000$.}
    \label{fig:converge:R07}
\end{figure*}

\begin{figure*}[!htb]
    \centering   
      \subfigure[(a) ImageNet]{
   \includegraphics[width = 0.18\columnwidth, trim=15 0 30 10, clip]{Figure/Converge/I08.eps}}
      \subfigure[(b) MNIST]{
   \includegraphics[width = 0.18\columnwidth, trim=15 0 30 10, clip]{Figure/Converge/M08.eps}}
      \subfigure[(c) PROTEIN]{
   \includegraphics[width = 0.18\columnwidth, trim=15 0 30 10, clip]{Figure/Converge/P08.eps}}
      \subfigure[(d) CIFAR]{ 
   \includegraphics[width = 0.18\columnwidth, trim=15 0 30 10, clip]{Figure/Converge/C08.eps}}
    \subfigure[(e) GoogleNews]{ 
   \includegraphics[width = 0.18\columnwidth, trim=15 0 30 10, clip]{Figure/Converge/G08.eps}}
   \caption{Tolerance on various datasets, with $m=1,000$ search candidates and $n=200$ query items, where missing ratio $\rho=0.8$, rank $r=100$, $\lambda = 0.001$, $\gamma=0.001$, iterations $T=10,000$.}
    \label{fig:converge:R08}
\end{figure*}

\begin{figure*}[!htb]
    \centering   
   
      \subfigure[(a) ImageNet]{
   \includegraphics[width = 0.18\columnwidth, trim=15 0 30 10, clip]{Figure/Converge/I09.eps}}
      \subfigure[(b) MNIST]{
   \includegraphics[width = 0.18\columnwidth, trim=15 0 30 10, clip]{Figure/Converge/M09.eps}}
      \subfigure[(c) PROTEIN]{
   \includegraphics[width = 0.18\columnwidth, trim=15 0 30 10, clip]{Figure/Converge/P09.eps}}
      \subfigure[(d) CIFAR]{ 
   \includegraphics[width = 0.18\columnwidth, trim=15 0 30 10, clip]{Figure/Converge/C09.eps}}
    \subfigure[(e) GoogleNews]{ 
   \includegraphics[width = 0.18\columnwidth, trim=15 0 30 10, clip]{Figure/Converge/G09.eps}}
   \caption{Tolerance on various datasets, with $m=1,000$ search candidates and $n=200$ query items, where missing ratio $\rho=0.9$, rank $r=100$, $\lambda = 0.001$, $\gamma=0.001$, iterations $T=10,000$.}
    \label{fig:converge:R09}
\end{figure*}


==> Figure/Time/AppTime.tex <==
\subsection{Efficiency Analysis}
\label{App:Time}
\begin{figure*}[!htb]
    \centering 
%      \subfigure[SIFT]{
%   \includegraphics[width = 0.19\columnwidth, trim=15 0 30 10, clip]{Figure/p05/SIFT05.eps}}
      \subfigure[(a) ImageNet]{
   \includegraphics[width = 0.19\columnwidth, trim=15 0 30 10, clip]{Figure/RankTime/p06/ImageNet06.eps}}
      \subfigure[(b) MNIST]{
   \includegraphics[width = 0.19\columnwidth, trim=15 0 30 10, clip]{Figure/RankTime/p06/MNIST06.eps}}
      \subfigure[(c) PROTEIN]{
   \includegraphics[width = 0.19\columnwidth, trim=15 0 30 10, clip]{Figure/RankTime/p06/PROTEIN06.eps}}
      \subfigure[(d) CIFAR]{ 
   \includegraphics[width = 0.19\columnwidth, trim=15 0 30 10, clip]{Figure/RankTime/p06/CIFAR06.eps}}
   \subfigure[(e) GoogleNews]{ 
   \includegraphics[width = 0.19\columnwidth, trim=15 0 30 10, clip]{Figure/RankTime/p06/Google06.eps}}
   \vspace{-0.4cm}
    \caption{Running Time versus rank $r$ on various dataset, with $m=1,000$ search candidates and $n=200$ query items, where missing ratio $\rho=0.6$, $\lambda = 0.001$, $\gamma = 0.001$, iterations $T=10,000$.}
    \label{fig:ranktime:p06}
\end{figure*}

\begin{figure*}[!htb]
    \centering 
%      \subfigure[SIFT]{
%   \includegraphics[width = 0.19\columnwidth, trim=15 0 30 10, clip]{Figure/p05/SIFT05.eps}}
      \subfigure[(a) ImageNet]{
   \includegraphics[width = 0.19\columnwidth, trim=15 0 30 10, clip]{Figure/RankTime/p07/ImageNet07.eps}}
      \subfigure[(b) MNIST]{
   \includegraphics[width = 0.19\columnwidth, trim=15 0 30 10, clip]{Figure/RankTime/p07/MNIST07.eps}}
      \subfigure[(c) PROTEIN]{
   \includegraphics[width = 0.19\columnwidth, trim=15 0 30 10, clip]{Figure/RankTime/p07/PROTEIN07.eps}}
      \subfigure[(d) CIFAR]{ 
   \includegraphics[width = 0.19\columnwidth, trim=15 0 30 10, clip]{Figure/RankTime/p07/CIFAR07.eps}}
   \subfigure[(e) GoogleNews]{ 
   \includegraphics[width = 0.19\columnwidth, trim=15 0 30 10, clip]{Figure/RankTime/p07/Google07.eps}}
   \vspace{-0.4cm}
    \caption{Running Time versus rank $r$ on various dataset, with $m=1,000$ search candidates and $n=200$ query items, where missing ratio $\rho=0.7$, $\lambda = 0.001$, $\gamma = 0.001$, iterations $T=10,000$.}
    \label{fig:ranktime:p07}
\end{figure*}

\begin{figure*}[!htb]
    \centering 
%      \subfigure[SIFT]{
%   \includegraphics[width = 0.19\columnwidth, trim=15 0 30 10, clip]{Figure/p05/SIFT05.eps}}
      \subfigure[(a) ImageNet]{
   \includegraphics[width = 0.19\columnwidth, trim=15 0 30 10, clip]{Figure/RankTime/p08/ImageNet08.eps}}
      \subfigure[(b) MNIST]{
   \includegraphics[width = 0.19\columnwidth, trim=15 0 30 10, clip]{Figure/RankTime/p08/MNIST08.eps}}
      \subfigure[(c) PROTEIN]{
   \includegraphics[width = 0.19\columnwidth, trim=15 0 30 10, clip]{Figure/RankTime/p08/PROTEIN08.eps}}
      \subfigure[(d) CIFAR]{ 
   \includegraphics[width = 0.19\columnwidth, trim=15 0 30 10, clip]{Figure/RankTime/p08/CIFAR08.eps}}
   \subfigure[(e) GoogleNews]{ 
   \includegraphics[width = 0.19\columnwidth, trim=15 0 30 10, clip]{Figure/RankTime/p08/Google08.eps}}
   \vspace{-0.4cm}
    \caption{Running Time versus rank $r$ on various dataset, with $m=1,000$ search candidates and $n=200$ query items, where missing ratio $\rho=0.8$, $\lambda = 0.001$, $\gamma = 0.001$, iterations $T=10,000$.}
    \label{fig:ranktime:p08}
\end{figure*}

\begin{figure*}[!htb]
    \centering 
%      \subfigure[SIFT]{
%   \includegraphics[width = 0.19\columnwidth, trim=15 0 30 10, clip]{Figure/p05/SIFT05.eps}}
      \subfigure[(a) ImageNet]{
   \includegraphics[width = 0.19\columnwidth, trim=15 0 30 10, clip]{Figure/RankTime/p09/ImageNet09.eps}}
      \subfigure[(b) MNIST]{
   \includegraphics[width = 0.19\columnwidth, trim=15 0 30 10, clip]{Figure/RankTime/p09/MNIST09.eps}}
      \subfigure[(c) PROTEIN]{
   \includegraphics[width = 0.19\columnwidth, trim=15 0 30 10, clip]{Figure/RankTime/p09/PROTEIN09.eps}}
      \subfigure[(d) CIFAR]{ 
   \includegraphics[width = 0.19\columnwidth, trim=15 0 30 10, clip]{Figure/RankTime/p09/CIFAR09.eps}} 
   \subfigure[(e) GoogleNews]{ 
   \includegraphics[width = 0.19\columnwidth, trim=15 0 30 10, clip]{Figure/RankTime/p09/Google09.eps}}
   \vspace{-0.4cm}
    \caption{Running Time versus rank $r$ on various dataset, with $m=1,000$ search candidates and $n=200$ query items, where missing ratio $\rho=0.9$, $\lambda = 0.001$, $\gamma = 0.001$, iterations $T=10,000$.}
    \label{fig:ranktime:p09}
\end{figure*}

 

%Convergence-DONE


==> Table/Ablation/DetailedAbla.tex <==
\begin{table}[!htb]
\centering
\huge
\caption{Comparisons of Various Ablation Methods, FrNorm denotes Frobenius Norm, NuNorm denotes Nuclear Norm. } 
\label{tab:RMSE:abmethodsall} 
\vspace{-0.4cm}
\resizebox{0.7\columnwidth}{!}{    
\begin{tabular}{ll|ll|l|l}
\toprule
\hline
\multicolumn{2}{c|}{\textbf{Methods}}                                                                                                                                         & \textbf{LoR} & \textbf{PSD} & \textbf{Regularizer} & \textbf{Solver}      \\ \hline
\multicolumn{1}{l|}{\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}SMC\\ Variants\\ (Regularizer)\end{tabular}}}} & \textbf{SMC\_F}                                      & ×            & $\checkmark$ & FrNorm               & Gradient Descent     \\
\multicolumn{1}{l|}{}                                                                                                 & \textbf{SMC\_NR}                                     & ×            & $\checkmark$ & No Regularizer       & Gradient Descent     \\
\multicolumn{1}{l|}{}                                                                                                 & \textbf{SMC\_GD}                                     & $\checkmark$ & $\checkmark$ & NuNorm               & Gradient Descent     \\ \hline
\multicolumn{1}{l|}{\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}SMC\\ Variants\\ (Solver)\end{tabular}}}}      & \textbf{SMC\_QN}                                     & $\checkmark$ & $\checkmark$ & No Regularizer       & Quasi Newton         \\
\multicolumn{1}{l|}{}                                                                                                 & \textbf{SMCNN\_QN}                                   & $\checkmark$ & $\checkmark$ & NuNorm               & Quasi Newton         \\
\multicolumn{1}{l|}{}                                                                                                 & \textbf{SMCNmF\_QN}                                  & $\checkmark$ & $\checkmark$ & NuNorm+FrNorm        & Quasi Newton         \\ \hline
\multicolumn{1}{l|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}MC\\ Variants\end{tabular}}}}                  & \textbf{MC\_ON}                                      & $\checkmark$ & ×            & NuNorm               & SVD Operation        \\
\multicolumn{1}{l|}{}                                                                                                 & \textbf{MC\_fON}                                     & $\checkmark$ & ×            & NuNorm               & Gradient Descent     \\ \hline
\multicolumn{1}{l|}{\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}PSD\\ SMC\end{tabular}}}}                      & \textbf{CMC}\cite{li2015estimating} & ×            & $\checkmark$ & No Regularizer       & Cyclic Projection    \\
\multicolumn{1}{l|}{}                                                                                                 & \textbf{DMC}\cite{li2020scalable}   & ×            & $\checkmark$ & No Regularizer       & Dykstra's Projection \\
\multicolumn{1}{l|}{}                                                                                                 & \textbf{FMC}\cite{ma2024fast}       & ×            & $\checkmark$ & No Regularizer       & Lagrangian Method    \\ \hline
\multicolumn{1}{l|}{\multirow{2}{*}{\textbf{OURS}}}                                                                   & \textbf{SMCNN (OURS)}                                & $\checkmark$ & $\checkmark$ & NuNorm               & Gradient Descent     \\
\multicolumn{1}{l|}{}                                                                                                 & \textbf{SMCNmF (OURS)}                               & $\checkmark$ & $\checkmark$ & NuNorm+FrNorm        & Gradient Descent     \\ \hline
\bottomrule
\end{tabular} 
}
\end{table}
 

==> Table/Ablation/Q2S1full.tex <==
\begin{table}[!htb]
\centering
\huge    
\caption{Ablation study on various variations of RMSE, Recall@top20\%, nDCG@top20\% with $m=1,000$ search candidates and $n=200$ query items, where missing ratio $\rho =\{0.7,0.8,0.9\}$, rank $r = 100$, $\lambda = 0.001$, $\gamma = 0.001$, and $T = 10,000$. The top 2 performances are highlighted in bold.} 
\label{tab:ab:Q2S1} 
\vspace{-0.4cm}
\resizebox{\columnwidth}{!}{   
\begin{tabular}{ll|lll|lll|lll}
\toprule
\hline
\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Dataset/Method}}}                                                     & \multicolumn{3}{c|}{\textbf{0.7}}                   & \multicolumn{3}{c|}{\textbf{0.8}}                   & \multicolumn{3}{c}{\textbf{0.9}}                    \\ \cline{3-11} 
\multicolumn{2}{c|}{}                                                                                             & \textbf{RMSE}   & \textbf{Recall} & \textbf{nDCG}   & \textbf{RMSE}   & \textbf{Recall} & \textbf{nDCG}   & \textbf{RMSE}   & \textbf{Recall} & \textbf{nDCG}   \\ \hline
\multicolumn{1}{l|}{\multirow{13}{*}{\textbf{ImageNet}}}   & \textbf{SMC\_F}                                      & 0.6496          & 0.5354          & 0.9602          & 0.5905          & 0.4521          & 0.6766          & 0.4586          & 0.7348          & 0.6750          \\
\multicolumn{1}{l|}{}                                      & \textbf{SMC\_NR}                                     & 0.6496          & 0.5375          & 0.9603          & 0.5904          & 0.4521          & 0.6745          & 0.4587          & 0.7348          & 0.6798          \\
\multicolumn{1}{l|}{}                                      & \textbf{SMC\_GD}                                     & 0.6122          & 0.6123          & 0.9469          & 0.4690          & 0.5170          & 0.6949          & 0.4574          & 0.7201          & 0.6329          \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                      & \textbf{SMC\_QN}                                     & 0.5845          & 0.4521          & 0.9575          & 0.5166          & 0.4396          & 0.6457          & 0.4566          & 0.7413          & 0.6470          \\
\multicolumn{1}{l|}{}                                      & \textbf{SMCNN\_QN}                                   & 0.5845          & 0.4521          & 0.9575          & 0.5166          & 0.4396          & 0.6366          & 0.4566          & 0.7422          & 0.6548          \\
\multicolumn{1}{l|}{}                                      & \textbf{SMCNmF\_QN}                                  & 0.5845          & 0.4521          & 0.9575          & 0.5166          & 0.4396          & 0.6426          & 0.4566          & 0.6426          & 0.6455          \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                      & \textbf{MC\_ON}                                      & 1.0120          & 0.5436          & 0.6475          & 1.5000          & 0.5663          & 0.6475          & 1.0830          & 0.4063          & 0.6476          \\
\multicolumn{1}{l|}{}                                      & \textbf{MC\_fON}                                     & 1.1602          & 0.6896          & 0.6553          & 0.6038          & 0.5217          & 0.6333          & 0.5169          & 0.5245          & 0.5672          \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                      & \textbf{CMC}\cite{li2015estimating} & 0.6539          & 0.7276          & 0.6772          & 0.5018          & 0.5280          & 0.5739          & 0.5462          & 0.7004          & 0.7988          \\
\multicolumn{1}{l|}{}                                      & \textbf{DMC}\cite{li2020scalable}   & 0.5980          & 0.6192          & 0.6320          & 0.4742          & 0.5915          & 0.6320          & 0.7714          & 0.6771          & 0.8290          \\
\multicolumn{1}{l|}{}                                      &  \textbf{FMC}\cite{ma2024fast}       & 0.6269          & 0.6644          & 0.6984          & 0.7347          & 0.4688          & 0.5984          & 0.7365          & 0.6613          & 0.8430          \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                      & \textbf{SMCNN(OURS)}                                 & \textbf{0.5689} & \textbf{0.8223} & \textbf{0.7866} & \textbf{0.4443} & \textbf{0.5951} & \textbf{0.6945} & \textbf{0.4546} & \textbf{0.7708} & \textbf{0.8951} \\
\multicolumn{1}{l|}{}                                      & \textbf{SMCNmF(OURS)}                                & \textbf{0.5658} & \textbf{0.8237} & \textbf{0.7992} & \textbf{0.4451} & \textbf{0.5950} & \textbf{0.6948} & \textbf{0.4457} & \textbf{0.7681} & \textbf{0.8952} \\ \hline
\multicolumn{1}{l|}{\multirow{13}{*}{\textbf{MNIST}}}      & \textbf{SMC\_F}                                      & 0.9721          & 0.6083          & 0.7628          & 0.8487          & 0.5396          & 0.7492          & 0.5682          & 0.4729          & 0.7346          \\
\multicolumn{1}{l|}{}                                      & \textbf{SMC\_NR}                                     & 0.9728          & 0.6083          & 0.7628          & 0.8488          & 0.5396          & 0.7490          & 0.5682          & 0.4729          & 0.7346          \\
\multicolumn{1}{l|}{}                                      & \textbf{SMC\_GD}                                     & 0.8380          & 0.7378          & 0.8155          & 0.7155          & 0.6156          & 0.7806          & 0.4913          & 0.6706          & 0.8429          \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                      & \textbf{SMC\_QN}                                     & 1.0310          & 0.6021          & 0.7635          & 0.8543          & 0.5313          & 0.7491          & 0.5676          & 0.4750          & 0.7353          \\
\multicolumn{1}{l|}{}                                      & \textbf{SMCNN\_QN}                                   & 1.0339          & 0.6042          & 0.7640          & 0.8565          & 0.5333          & 0.7488          & 0.5681          & 0.4750          & 0.7353          \\
\multicolumn{1}{l|}{}                                      & \textbf{SMCNmF\_QN}                                  & 1.0416          & 0.6083          & 0.7644          & 0.8515          & 0.5333          & 0.7488          & 0.5681          & 0.4750          & 0.7353          \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                      & \textbf{MC\_ON}                                      & 0.8878          & 0.6577          & 0.7707          & 0.7415          & 0.5440          & 0.7226          & 0.7377          & 0.5177          & 0.7707          \\
\multicolumn{1}{l|}{}                                      & \textbf{MC\_fON}                                     & 0.9593          & 0.6236          & 0.7780          & 0.7416          & 0.5440          & 0.7726          & 0.7377          & 0.5317          & 0.7707          \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                      & \textbf{CMC}\cite{li2015estimating} & 1.0000          & 0.6285          & 0.7095          & 0.9962          & 0.5525          & 0.7291          & 0.7788          & 0.6604          & 0.8314          \\
\multicolumn{1}{l|}{}                                      & \textbf{DMC}\cite{li2020scalable}   & 1.0774          & 0.6025          & 0.7409          & 0.7513          & 0.5103          & 0.7409          & 0.5378          & 0.6617          & 0.8125          \\
\multicolumn{1}{l|}{}                                      &  \textbf{FMC}\cite{ma2024fast}       & 0.8491          & 0.6840          & 0.7998          & \textbf{0.6559} & 0.5645          & 0.7065          & 0.6573          & 0.6451          & 0.7977          \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                      & \textbf{SMCNN(OURS)}                                 & \textbf{0.8233} & \textbf{0.7762} & \textbf{0.8488} & \textbf{0.7080} & \textbf{0.6432} & \textbf{0.7845} & \textbf{0.4893} & \textbf{0.6961} & \textbf{0.8854} \\
\multicolumn{1}{l|}{}                                      & \textbf{SMCNmF(OURS)}                                & \textbf{0.8236} & \textbf{0.7762} & \textbf{0.8542} & 0.7115          & \textbf{0.6323} & \textbf{0.7829} & \textbf{0.4893} & \textbf{0.6961} & \textbf{0.8814} \\ \hline
\multicolumn{1}{l|}{\multirow{13}{*}{\textbf{PROTEIN}}}    & \textbf{SMC\_F}                                      & 0.7829          & 0.6448          & 0.7970          & 0.7178          & 0.4437          & 0.6580          & 0.6078          & 0.5979          & 0.7914          \\
\multicolumn{1}{l|}{}                                      & \textbf{SMC\_NR}                                     & 0.7853          & 0.6586          & 0.7969          & 0.7191          & 0.4357          & 0.6548          & 0.6076          & 0.6021          & 0.7914          \\
\multicolumn{1}{l|}{}                                      & \textbf{SMC\_GD}                                     & 0.5922          & 0.7613          & 0.7775          & 0.5177          & 0.5178          & 0.7455          & 0.5291          & 0.7284          & 0.8864          \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                      & \textbf{SMC\_QN}                                     & 1.1635          & 0.5428          & 0.7898          & 0.7028          & 0.4604          & 0.6565          & 0.5458          & 0.4250          & 0.7879          \\
\multicolumn{1}{l|}{}                                      & \textbf{SMCNN\_QN}                                   & 1.1645          & 0.5648          & 0.7898          & 0.7027          & 0.4604          & 0.6500          & 0.5463          & 0.4250          & 0.7879          \\
\multicolumn{1}{l|}{}                                      & \textbf{SMCNmF\_QN}                                  & 1.1646          & 0.5558          & 0.7898          & 0.7027          & 0.4604          & 0.6565          & 0.5462          & 0.4250          & 0.7879          \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                      & \textbf{MC\_ON}                                      & 0.9221          & 0.5448          & 0.6605          & 0.7797          & 0.9304          & 0.6536          & 0.5730          & 0.7693          & 0.8233          \\
\multicolumn{1}{l|}{}                                      & \textbf{MC\_fON}                                     & 1.1450          & 0.4997          & 0.6705          & 0.7448          & 0.9244          & 0.6313          & 0.6780          & 0.7692          & 0.8332          \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                      & \textbf{CMC}\cite{li2015estimating} & 0.7731          & 0.5980          & 0.7970          & 0.5946          & 0.4515          & 0.6436          & 0.5241          & 0.7614          & 0.8954          \\
\multicolumn{1}{l|}{}                                      & \textbf{DMC}\cite{li2020scalable}   & 0.8329          & 0.6029          & 0.7548          & 0.6585          & 0.4990          & 0.6548          & 0.5136          & 0.7455          & 0.8959          \\
\multicolumn{1}{l|}{}                                      &  \textbf{FMC}\cite{ma2024fast}       & 0.6313          & 0.6772          & 0.6995          & 0.5665          & 0.5618          & 0.6995          & 0.5664          & 0.6715          & 0.8949          \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                      & \textbf{SMCNN(OURS)}                                 & \textbf{0.5861} & \textbf{0.7435} & \textbf{0.7974} & \textbf{0.4885} & \textbf{0.5160} & \textbf{0.6955} & \textbf{0.5049} & \textbf{0.7814} & \textbf{0.9255} \\
\multicolumn{1}{l|}{}                                      & \textbf{SMCNmF(OURS)}                                & \textbf{0.5832} & \textbf{0.7649} & \textbf{0.7974} & \textbf{0.4887} & \textbf{0.5240} & \textbf{0.6955} & \textbf{0.5049} & \textbf{0.7814} & \textbf{0.9436} \\ \hline
\multicolumn{1}{l|}{\multirow{13}{*}{\textbf{CIFAR}}}      & \textbf{SMC\_F}                                      & 0.9999          & 0.5442          & 0.7783          & 0.9798          & 0.5479          & 0.6548          & 0.8367          & 0.4604          & 0.7614          \\
\multicolumn{1}{l|}{}                                      & \textbf{SMC\_NR}                                     & 1.0000          & 0.5463          & 0.7783          & 0.9801          & 0.5458          & 0.6458          & 0.8369          & 0.4604          & 0.7614          \\
\multicolumn{1}{l|}{}                                      & \textbf{SMC\_GD}                                     & 0.7380          & 0.6378          & 0.8594          & 0.5594          & 0.6595          & 0.6270          & 0.5698          & 0.7589          & 0.8234          \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                      & \textbf{SMC\_QN}                                     & 1.3499          & 0.5321          & 0.7748          & 1.1460          & 0.5083          & 0.6458          & 0.8539          & 0.4458          & 0.7618          \\
\multicolumn{1}{l|}{}                                      & \textbf{SMCNN\_QN}                                   & 1.3500          & 0.4532          & 0.7750          & 1.1435          & 0.5104          & 0.6458          & 0.8512          & 0.4479          & 0.7618          \\
\multicolumn{1}{l|}{}                                      & \textbf{SMCNmF\_QN}                                  & 1.3498          & 0.5542          & 0.7750          & 1.1361          & 0.5083          & 0.6548          & 0.8556          & 0.4458          & 0.7618          \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                      & \textbf{MC\_ON}                                      & 0.9226          & 0.5358          & 0.6530          & 0.7815          & 0.5693          & 0.6546          & 0.5729          & 0.5693          & 0.8543          \\
\multicolumn{1}{l|}{}                                      & \textbf{MC\_fON}                                     & 0.9226          & 0.5558          & 0.6510          & 0.7815          & 0.5930          & 0.6209          & 0.5729          & 0.5436          & 0.8435          \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                      & \textbf{CMC}\cite{li2015estimating} & 0.9887          & 0.6284          & 0.8622          & 0.7288          & 0.6244          & 0.6123          & 0.5214          & 0.7314          & 0.8248          \\
\multicolumn{1}{l|}{}                                      & \textbf{DMC}\cite{li2020scalable}   & 1.0430          & 0.5893          & 0.8379          & 0.5747          & 0.6309          & 0.6379          & 0.5145          & 0.7251          & 0.8483          \\
\multicolumn{1}{l|}{}                                      &  \textbf{FMC}\cite{ma2024fast}       & 0.5459          & 0.5775          & 0.6977          & 0.6509          & 0.5775          & 0.5995          & 0.5269          & 0.7274          & 0.7977          \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                      & \textbf{SMCNN(OURS)}                                 & \textbf{0.7044} & \textbf{0.6832} & \textbf{0.8903} & \textbf{0.5097} & \textbf{0.6822} & \textbf{0.6878} & \textbf{0.4239} & \textbf{0.7491} & \textbf{0.8658} \\
\multicolumn{1}{l|}{}                                      & \textbf{SMCNmF(OURS)}                                & \textbf{0.7044} & \textbf{0.6832} & \textbf{0.8913} & \textbf{0.5081} & \textbf{0.6842} & \textbf{0.6819} & \textbf{0.4239} & \textbf{0.7492} & \textbf{0.8686} \\ \hline
\multicolumn{1}{l|}{\multirow{13}{*}{\textbf{GoogleNews}}} & \textbf{SMC\_F}                                      & 0.8612          & 0.6553          & 0.7930          & 0.7754          & 0.6598          & 0.6790          & 0.6395          & 0.6771          & 0.7736          \\
\multicolumn{1}{l|}{}                                      & \textbf{SMC\_NR}                                     & 0.8603          & 0.6554          & 0.7930          & 0.7754          & 0.6370          & 0.6899          & 0.6394          & 0.6771          & 0.7736          \\
\multicolumn{1}{l|}{}                                      & \textbf{SMC\_GD}                                     & 0.6024          & 0.7051          & 0.8019          & 0.5219          & 0.7087          & 0.6778          & 0.5617          & 0.7216          & 0.8374          \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                      & \textbf{SMC\_QN}                                     & 0.8348          & 0.6433          & 0.7937          & 0.7689          & 0.6537          & 0.6368          & 0.6451          & 0.6534          & 0.7730          \\
\multicolumn{1}{l|}{}                                      & \textbf{SMCNN\_QN}                                   & 0.8353          & 0.6234          & 0.7937          & 0.7693          & 0.6548          & 0.6537          & 0.6454          & 0.6534          & 0.7724          \\
\multicolumn{1}{l|}{}                                      & \textbf{SMCNmF\_QN}                                  & 0.8352          & 0.6643          & 0.7937          & 0.7693          & 0.6785          & 0.6438          & 0.6453          & 0.6345          & 0.7724          \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                      & \textbf{MC\_ON}                                      & 0.8425          & 0.6423          & 0.6301          & 0.7595          & 0.6458          & 0.6532          & 0.5768          & 0.6436          & 0.7354          \\
\multicolumn{1}{l|}{}                                      & \textbf{MC\_fON}                                     & 0.8433          & 0.6345          & 0.5907          & 0.7597          & 0.6548          & 0.6362          & 0.5769          & 0.6565          & 0.7354          \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                      & \textbf{CMC}\cite{li2015estimating} & 0.8085          & 0.6175          & 0.7989          & 0.5776          & 0.6138          & 0.6985          & 0.7141          & 0.7241          & 0.8848          \\
\multicolumn{1}{l|}{}                                      & \textbf{DMC}\cite{li2020scalable}   & 0.9477          & 0.6340          & 0.7950          & 0.5231          & 0.6134          & 0.6950          & 0.5645          & 0.6600          & 0.7984          \\
\multicolumn{1}{l|}{}                                      &  \textbf{FMC}\cite{ma2024fast}       & 0.6109          & 0.7075          & 0.7998          & 0.5362          & 0.6743          & 0.6843          & 0.5322          & 0.6743          & 0.6949          \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                      & \textbf{SMCNN(OURS)}                                 & \textbf{0.5553} & \textbf{0.7366} & \textbf{0.8170} & \textbf{0.4241} & \textbf{0.7129} & \textbf{0.6980} & \textbf{0.5115} & \textbf{0.7685} & \textbf{0.8922} \\
\multicolumn{1}{l|}{}                                      & \textbf{SMCNmF(OURS)}                                & \textbf{0.5684} & \textbf{0.7364} & \textbf{0.8130} & \textbf{0.4232} & \textbf{0.7120} & \textbf{0.6980} & \textbf{0.5116} & \textbf{0.7686} & \textbf{0.8958} \\ \hline
\bottomrule
\end{tabular} 
}
\end{table}

==> Table/Ablation/Q2S2.tex <==
\begin{table*}[!htb] 
\centering
\scriptsize 
\caption{Ablation study on various variations of RMSE, Recall@top20\%, nDCG@top20\% with $m=2,000$ search candidates and $n=200$ query items, where missing ratio $\rho =\{0.7,0.8,0.9\}$, rank $r = 100$, $\lambda = 0.001$, $\gamma = 0.001$, and $T = 10,000$. The top 2 performances are highlighted in bold.} 
\label{tab:ab:Q2S2} 
\resizebox{0.9\columnwidth}{!}{ 
\begin{tabular}{ll|lll|lll|lll}
\toprule
\hline
\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Dataset/Method}}}                      & \multicolumn{3}{c|}{\textbf{0.7}}                   & \multicolumn{3}{c|}{\textbf{0.8}}                   & \multicolumn{3}{c}{\textbf{0.9}}                    \\   \cline{3-11} 
\multicolumn{2}{c|}{}          & \textbf{RMSE}   & \textbf{Recall} & \textbf{nDCG}   & \textbf{RMSE}   & \textbf{Recall} & \textbf{nDCG}   & \textbf{RMSE}   & \textbf{Recall} & \textbf{nDCG}   \\ \hline
\multicolumn{1}{l|}{\multirow{13}{*}{\textbf{ImageNet}}}  & \textbf{SMC\_F}    & 0.7169          & 0.6583          & 0.7955          & 0.6927          & 0.6729          & 0.7770          & 0.6546          & 0.6235          & 0.7655          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_NR}    & 0.7162          & 0.6583          & 0.7954          & 0.6926          & 0.6729          & 0.7770          & 0.6345          & 0.6254          & 0.7547          \\ 
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_GD} & 0.7390 & 0.7365 & 0.7699 & 0.6699 & 0.7100 & 0.8202 & 0.6199 & 0.6264 & 0.7264  \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_QN}    & 0.6991          & 0.5364          & 0.7899          & 0.6961          & 0.6604          & 0.7774          & 0.6345          & 0.6245          & 0.7457          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNN\_QN}    & 0.6995          & 0.5344          & 0.7899          & 0.6964          & 0.6604          & 0.7774          & 0.6549          & 0.5865          & 0.7655          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNmF\_QN}    & 0.6994          & 0.4438          & 0.7899          & 0.6964          & 0.6604          & 0.7774          & 0.6547          & 0.5645          & 0.7565          \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                     & \textbf{MC\_ON}    & 0.6405          & 0.6549          & 0.7359          & 0.8791          & 0.6348          & 0.7541          & 0.6370          & 0.5264          & 0.7228          \\
\multicolumn{1}{l|}{}                                     & \textbf{MC\_fON}    & 0.6406          & 0.6439          & 0.7457          & 0.8791          & 0.6542          & 0.7453          & 0.6377          & 0.5546          & 0.7690          \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                     & \textbf{CMC} \cite{li2015estimating}        & 0.7199          & 0.7320          & 0.8213          & 0.7808          & 0.6572          & 0.8546          & 0.6779          & 0.6604          & \textbf{0.8984} \\
\multicolumn{1}{l|}{}                                     & \textbf{DMC} \cite{li2020scalable}         & 0.7094          & 0.7293          & 0.8410          & 0.7090          & 0.6715          & 0.8652          & 0.6538          & 0.6617          & 0.8541          \\
\multicolumn{1}{c|}{}                                    & \textbf{SMC} \cite{ma2024fast}    & 0.6987                    & 0.5157                     & 0.7000                     & 0.6981                     & 0.5945                     & 0.7000                     & 0.6934 & 0.7932 & 0.7000 \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{SMCNN (OURS)}        & \textbf{0.6682} & \textbf{0.7896} & \textbf{0.8912} & \textbf{0.5665} & \textbf{0.7208} & \textbf{0.8994} & \textbf{0.5815} & \textbf{0.6917} & \textbf{0.8979} \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNmF (OURS)}       & \textbf{0.6581} & \textbf{0.7958} & \textbf{0.8923} & \textbf{0.5667} & \textbf{0.7250} & \textbf{0.8949} & \textbf{0.5856} & \textbf{0.6981} & 0.8778 \\ \hline 
\multicolumn{1}{l|}{\multirow{13}{*}{\textbf{MNIST}}}     & \textbf{SMC\_F}    & 0.8163          & 0.6745          & 0.6578          & 0.7552          & 0.6542          & 0.7763          & 0.5402          & 0.3563          & 0.6772          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_NR}    & 0.8160          & 0.6467          & 0.6979          & 0.7551          & 0.6542          & 0.7456          & 0.5542          & 0.3563          & 0.6717          \\ 
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_GD} & 0.7413 & 0.7018 & 0.7239 & 0.6759 & 0.7340 & 0.8314 & 0.6311 & 0.7281 & 0.8281 \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_QN}    & 0.8281          & 0.6766          & 0.6862          & 0.7443          & 0.6764          & 0.7643          & 0.5760          & 0.3583          & 0.6718          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNN\_QN}    & 0.8287          & 0.6866          & 0.6869          & 0.7448          & 0.6542          & 0.7765          & 0.5770          & 0.3583          & 0.6177          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNmF\_QN}    & 0.8287          & 0.6866          & 0.6857          & 0.7447          & 0.5464          & 0.7765          & 0.5654          & 0.6536          & 0.7177          \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                     & \textbf{MC\_ON}    & 0.7435          & 0.6456          & 0.6547          & 0.6401          & 0.6746          & 0.7659          & 0.5634          & 0.6913          & 0.0320          \\
\multicolumn{1}{l|}{}                                     & \textbf{MC\_fON}    & 0.7306          & 0.6467          & 0.6452          & 0.6655          & 0.6869          & 0.7654          & 0.7544          & 0.6346          & 0.7343          \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                     & \textbf{CMC} \cite{li2015estimating}        & 0.8000          & 0.6849          & 0.6894          & 0.6815          & 0.7135          & 0.8420          & 0.5241          & 0.7614          & 0.8543          \\
\multicolumn{1}{l|}{}                                     & \textbf{DMC} \cite{li2020scalable}         & 0.7607          & 0.6842          & 0.6895          & 0.6726          & 0.7190          & 0.8452          & 0.5136          & 0.7455          & 0.8324          \\ 
\multicolumn{1}{c|}{}                                      & \textbf{SMC} \cite{ma2024fast}  & 0.7945                     & \textbf{0.7282}                     & 0.8295                     & \textbf{0.6658}                     & 0.7148                     & 0.8748                     & 0.6398 & \textbf{0.7921} & 0.7997 \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{SMCNN (OURS)}        & \textbf{0.7299} & 0.6938 & \textbf{0.7156} & \textbf{0.6703} & \textbf{0.7384} & \textbf{0.8954} & \textbf{0.5049} & \textbf{0.7814} & \textbf{0.8954} \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNmF (OURS)}       & \textbf{0.7257} & \textbf{0.7063} & \textbf{0.7086} & \textbf{0.6703} & \textbf{0.7383} & \textbf{0.8965} & \textbf{0.5049} & \textbf{0.7814} & \textbf{0.8965} \\ \hline 
\multicolumn{1}{l|}{\multirow{13}{*}{\textbf{PROTEIN}}}   & \textbf{SMC\_F}    & 0.7486          & 0.5779          & 0.7276          & 0.7555          & 0.6510          & 0.6555          & 0.6650          & 0.7152          & 0.6733          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_NR}    & 0.7486          & 0.5679          & 0.7263          & 0.7551          & 0.6544          & 0.6457          & 0.6535          & 0.7021          & 0.6733          \\ 
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_GD} & 0.7472 & 0.6756 & 0.7461 & 0.6861 & 0.7262 & 0.6406 & 0.6406 & 0.7264 & 0.8726 \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_QN}    & 0.7490          & 0.5683          & 0.7264          & 0.7548          & 0.6744          & 0.6650          & 0.6505          & 0.6935          & 0.6704          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNN\_QN}    & 0.7492          & 0.5758          & 0.7264          & 0.7555          & 0.6454          & 0.6646          & 0.6505          & 0.6955          & 0.6704          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNmF\_QN}    & 0.7492          & 0.5783          & 0.7254          & 0.7550          & 0.6454          & 0.6750          & 0.6748          & 0.6852          & 0.6704          \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                     & \textbf{MC\_ON}    & 0.7439          & 0.5769          & 0.7352          & 0.6401          & 0.6492          & 0.6487          & 0.6540          & 0.6791          & 0.7013          \\
\multicolumn{1}{l|}{}                                     & \textbf{MC\_fON}    & 0.7439          & 0.5774          & 0.7246          & 0.6401          & 0.6452          & 0.6469          & 0.6540          & 0.6591          & 0.7032          \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                     & \textbf{CMC} \cite{li2015estimating}        & 0.7531          & 0.6431          & 0.6851          & 0.6753          & 0.6841          & 0.6799          & 0.6521          & 0.6314          & 0.7865          \\
\multicolumn{1}{l|}{}                                     & \textbf{DMC} \cite{li2020scalable}         & 0.7470          & 0.6352          & 0.8953          & 0.6753          & 0.7066          & 0.6835          & 0.6515          & 0.6251          & 0.7843          \\  
\multicolumn{1}{c|}{}                                     & \textbf{SMC} \cite{ma2024fast}  &  0.7506                     & \textbf{0.6924}                     & 0.6989                     & 0.6820                     & 0.7056                     & 0.7430                     & 0.6358 & 0.7292 & 0.7997 \\ \cline{2-11}  
\multicolumn{1}{l|}{}                                     & \textbf{SMCNN (OURS)}        & \textbf{0.7280} & \textbf{0.6652} & \textbf{0.7978} & \textbf{0.6589} & \textbf{0.7167} & \textbf{0.6983} & \textbf{0.6152} & \textbf{0.7367} & \textbf{0.8792} \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNmF (OURS)}       & \textbf{0.7256} & 0.6588 & \textbf{0.7467} & \textbf{0.6465} & \textbf{0.7375} & \textbf{0.6987} & \textbf{0.6170} & \textbf{0.7383} & \textbf{0.8734} \\ \hline 
\multicolumn{1}{l|}{\multirow{13}{*}{\textbf{CIFAR10}}}     & \textbf{SMC\_F}    & 0.8169          & 0.6565          & 0.6550          & 0.7398          & 0.6549          & 0.7924          & 0.6841          & 0.6445          & 0.7844          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_NR}    & 0.8162          & 0.6555          & 0.6554          & 0.7639          & 0.6549          & 0.7924          & 0.6684          & 0.6435          & 0.7843          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_GD} & 0.6661 & 0.7075 & 0.7811 & 0.6661 & 0.7162 & 0.8080 & 0.6081 & 0.6040 & 0.8040 \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_QN}    & 0.8001          & 0.6545          & 0.6592          & 0.7540          & 0.6473          & 0.7900          & 0.6742          & 0.6535          & 0.7842          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNN\_QN}    & 0.8005          & 0.6565          & 0.6432          & 0.7541          & 0.6545          & 0.7900          & 0.6418          & 0.6374          & 0.7842          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNmF\_QN}    & 0.8005          & 0.6544          & 0.7147          & 0.7541          & 0.6547          & 0.7900          & 0.6841          & 0.6444          & 0.7984          \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                     & \textbf{MC\_ON}    & 0.7516          & 0.6543          & 0.7758          & 0.6411          & 0.6452          & 0.7859          & 0.6033          & 0.6391          & 0.7317          \\
\multicolumn{1}{l|}{}                                     & \textbf{MC\_fON}    & 0.7517          & 0.6575          & 0.7348          & 0.6412          & 0.6452          & 0.7786          & 0.6043          & 0.6391          & 0.7762          \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                     & \textbf{CMC} \cite{li2015estimating}        & 0.8614          & 0.7041          & 0.7410          & 0.8892          & 0.6948          & 0.7850          & 0.7141          & 0.6241          & 0.7984          \\
\multicolumn{1}{l|}{}                                     & \textbf{DMC} \cite{li2020scalable}         & 0.8659          & 0.7051          & 0.7530          & 0.7146          & \textbf{0.7324}          & \textbf{0.8542}          & 0.6245          & 0.6600          & 0.7854          \\
\multicolumn{1}{c|}{}                                      & \textbf{SMC} \cite{ma2024fast}  & 0.7711                     & 0.6330                     & 0.7230                     & 0.7977                     & 0.7049                     & 0.6713                     & 0.6297 & \textbf{0.7021} & \textbf{0.8415} \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                     & \textbf{SMCNN (OURS)}        & \textbf{0.6410} & \textbf{0.7165} & \textbf{0.7721} & \textbf{0.6600} & \textbf{0.7188} & \textbf{0.8019} & \textbf{0.5915} & \textbf{0.6646} & \textbf{0.7973} \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNmF (OURS)}       & \textbf{0.6533} & \textbf{0.7192} & \textbf{0.7802} & \textbf{0.6752} & 0.7130 & 0.8014 & \textbf{0.5933} & 0.6500 & 0.7971 \\ \hline 
\multicolumn{1}{l|}{\multirow{13}{*}{\textbf{GoogleNews}}} & \textbf{SMC\_F}    & 0.7803          & 0.5380          & 0.7581          & 0.7879          & 0.5899          & 0.7084          & 0.7185          & 0.7881          & 0.6786          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_NR}    & 0.7827          & 0.5438          & 0.7581          & 0.7873          & 0.5992          & 0.7087          & 0.7096          & 0.7854          & 0.6785          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_GD} & 0.7313 & 0.6304 & 0.6919 & 0.6945 & 0.6219 & 0.6202 & 0.6221 & 0.8131 & 0.8131  \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_QN}    & 1.1029          & 0.5434          & 0.7550          & 0.8145          & 0.5892          & 0.7296          & 0.6545          & 0.7544          & 0.6496          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNN\_QN}    & 1.1029          & 0.5434          & 0.7550          & 0.8145          & 0.5784          & 0.6970          & 0.6552          & 0.7544          & 0.6496          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNmF\_QN}    & 1.1028          & 0.5564          & 0.7550          & 0.7146          & 0.5629          & 0.6987          & 0.6552          & 0.7564          & 0.6550          \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                     & \textbf{MC\_ON}    & 1.0831          & 0.5165          & 0.6735          & 0.7000          & 0.6110          & 0.6766          & 0.6552          & 0.7540          & 0.6755          \\
\multicolumn{1}{l|}{}                                     & \textbf{MC\_fON}    & 1.0044          & 0.5285          & 0.6392          & 1.1601          & 0.6277          & 0.6987          & 0.6752          & 0.6760          & 0.6919          \\ \cline{2-11} 
\multicolumn{1}{l|}{}                                     & \textbf{CMC} \cite{li2015estimating}        & 0.7107          & 0.5500          & 0.6451          & 0.8693          & 0.4250          & 0.6869          & 0.8404          & 0.7378          & 0.7555          \\
\multicolumn{1}{l|}{}                                     & \textbf{DMC} \cite{li2020scalable}         & 0.7354          & \textbf{0.5608}          & 0.6495          & 0.8692          & 0.5021          & 0.6913          & 0.8227          & 0.7386          & 0.7955          \\
\multicolumn{1}{c|}{}                                     & \textbf{SMC} \cite{ma2024fast}   &   \textbf{0.6870}  &  \textbf{0.7009} &  \textbf{0.7190}  &  0.7654  &  0.7014  &  0.7997 & 0.6203 & 0.7012 & 0.7090 \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{SMCNN (OURS)}        & \textbf{0.6880} & 0.5496 & \textbf{0.7194} & \textbf{0.6208} & \textbf{0.6369} & \textbf{0.7242} & \textbf{0.6179} & \textbf{0.8381} & \textbf{0.8569} \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNmF (OURS)}       & 0.7083 & 0.5521 & 0.7183 & \textbf{0.6237} & \textbf{0.6429} & \textbf{0.7270} & \textbf{0.6096} & \textbf{0.8354} & \textbf{0.8502} \\ \hline
\bottomrule
\end{tabular} 
}
\end{table*}

==> Table/Ablation/Q2S3.tex <==
\begin{table*}[!htb] 
\centering
\scriptsize 
\caption{Ablation study on various variations of RMSE, Recall@top20\%, nDCG@top20\% with $m=3,000$ search candidates and $n=200$ query items, where missing ratio $\rho =\{0.7,0.8,0.9\}$, rank $r = 100$, $\lambda = 0.001$, $\gamma = 0.001$, and $T = 10,000$. The top 2 performances are highlighted in bold.} 
\label{tab:ab:Q2S3} 
\resizebox{0.9\columnwidth}{!}{ 
\begin{tabular}{ccc|ccc|ccc|ccc}
\toprule
\hline
\multicolumn{3}{c|}{\multirow{2}{*}{\textbf{Dataset/Method}}}                                                                      & \multicolumn{3}{c|}{\textbf{0.7}}                   & \multicolumn{3}{c|}{\textbf{0.8}}                   & \multicolumn{3}{c}{\textbf{0.9}}                    \\ \cline{4-12} 
\multicolumn{3}{c|}{}                                                                                                              & \textbf{RMSE}   & \textbf{Recall} & \textbf{nDCG}   & \textbf{RMSE}   & \textbf{Recall} & \textbf{nDCG}   & \textbf{RMSE}   & \textbf{Recall} & \textbf{nDCG}   \\ \hline
\multicolumn{1}{c|}{\multirow{12}{*}{\textbf{GoogleNews}}} & \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{MVI}}} & \textbf{MEAN}    & 1.2304          & 0.7172          & 0.7849          & 1.1189          & 0.6905          & 0.8178          & 1.0655          & 0.6582          & 0.6775          \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              & \textbf{LR}      & 1.3688          & 0.6573          & 0.7639          & 1.1774          & 0.6436          & 0.7404          & 1.1036          & 0.6291          & 0.6717          \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              & \textbf{GR}      & 1.4860          & 0.6677          & 0.7850          & 2.3145          & 0.6348          & 0.7455          & 3.1756          & 0.6116          & 0.6712          \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              & \textbf{KFMC}    & 1.3280          & 0.6787          & 0.7043          & 1.1758          & 0.6499          & 0.7720          & 2.1283          & 0.6115          & 0.6735          \\ \cline{2-12} 
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{MF}}}  & \textbf{FGSR}    & 1.5632          & 0.6858          & 0.7543          & 1.1230          & 0.6754          & 0.8942          & 1.5241          & 0.6724          & 0.6775          \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              & \textbf{BPMF}    & 1.1243          & 0.6833          & 0.7653          & 1.5420          & 0.5234          & 0.8543          & 1.4321          & 0.6782          & 0.6580          \\ \cline{2-12} 
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{PSD}}} & \textbf{CMC}     & 0.8931          & 0.6853          & 0.7231          & 0.8117          & 0.5897          & 0.8693          & 0.5987          & 0.6640          & 0.6812          \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              & \textbf{DMC}     & 0.7922          & 0.6898          & 0.7933          & 0.7452          & 0.5963          & 0.8954          & 0.5690          & 0.6872          & 0.6843          \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              &  \textbf{FMC}\cite{ma2024fast}     & 0.8958          & 0.6919          & 0.7999          & 0.8493          & 0.6908          & 0.7280          & 0.6269          & 0.6644          & 0.6843          \\ \cline{2-12} 
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{LR}}}  & \textbf{NNFN}    & 1.4652          & 0.6006          & 0.8643          & 0.8431          & 0.5906          & 0.7540          & 0.5883          & 0.5902          & 0.6854          \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              & \textbf{facNNFN} & 1.5710          & 0.6090          & 0.8944          & 1.5550          & 0.6209          & 0.7644          & 0.8750          & 0.6209          & 0.6530          \\ \cline{2-12} 
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{OUR}}} & \textbf{SSNN}    & \textbf{0.7821} & \textbf{0.7080} & \textbf{0.8900} & \textbf{0.6645} & \textbf{0.7630} & \textbf{0.7960} & \textbf{0.5444} & \textbf{0.7125} & \textbf{0.6897} \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              & \textbf{SSNmF}   & \textbf{0.7823} & \textbf{0.7354} & \textbf{0.8569} & \textbf{0.6707} & \textbf{0.7594} & \textbf{0.7963} & \textbf{0.5426} & \textbf{0.7229} & \textbf{0.6928} \\ \hline
\multicolumn{1}{c|}{\multirow{12}{*}{\textbf{ImageNet}}}   & \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{MVI}}} & \textbf{MEAN}    & 6.7102          & 0.5280          & 0.6962          & 4.4416          & 0.4547          & 0.5812          & 1.5308          & 0.5380          & 0.7935          \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              & \textbf{LR}      & 1.2252          & 0.5811          & 0.6961          & 1.5743          & 0.7981          & 0.5776          & 1.1619          & 0.5754          & 0.7918          \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              & \textbf{GR}      & 1.8592          & 0.5701          & 0.6963          & 1.1309          & 0.6521          & 0.5760          & 2.3223          & 0.4613          & 0.7917          \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              & \textbf{KFMC}    & 1.7922          & 0.5764          & 0.6892          & 1.3898          & 0.6809          & 0.7083          & 2.6780          & 0.5397          & 0.7919          \\ \cline{2-12} 
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{MF}}}  & \textbf{FGSR}    & 1.7250          & \textbf{0.6990} & 0.6807          & 1.6170          & \textbf{0.6990} & 0.7074          & 1.7776          & 0.5299          & 0.7807          \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              & \textbf{BPMF}    & 1.4200          & \textbf{0.6914} & 0.6893          & 1.5600          & 0.6286          & 0.6923          & 2.8260          & 0.5314          & 0.7897          \\ \cline{2-12} 
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{PSD}}} & \textbf{CMC}     & 0.9073          & 0.6580          & 0.6896          & 0.6322          & 0.6237          & 0.6893          & 0.6180          & 0.6360          & 0.7841          \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              & \textbf{DMC}     & 0.7411          & 0.6280          & 0.6886          & 0.6391          & 0.6220          & 0.6862          & 0.5983          & 0.6474          & 0.7854          \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              &  \textbf{FMC}\cite{ma2024fast}     & 0.5789          & 0.6196          & 0.6661          & 0.7301          & 0.6717          & 0.6997          & 0.6109          & 0.6175          & 0.7654          \\ \cline{2-12} 
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{LR}}}  & \textbf{NNFN}    & 0.6366          & 0.6091          & 0.6863          & 0.6997          & 0.6790          & 0.6763          & 0.7661          & 0.5619          & 0.7854          \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              & \textbf{facNNFN} & 1.2193          & 0.5927          & 0.6876          & 3.7254          & 0.5678          & 0.6764          & 3.2501          & 0.6030          & 0.7923          \\ \cline{2-12} 
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{OUR}}} & \textbf{SSNN}    & \textbf{0.5762} & 0.6230          & \textbf{0.6921} & \textbf{0.6106} & 0.6719          & \textbf{0.7648} & \textbf{0.5955} & \textbf{0.6517} & \textbf{0.7948} \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              & \textbf{SSNmF}   & \textbf{0.5675} & 0.6245          & \textbf{0.6922} & \textbf{0.6140} & \textbf{0.6775} & \textbf{0.7616} & \textbf{0.5864} & \textbf{0.6583} & \textbf{0.7964} \\ \hline
\multicolumn{1}{c|}{\multirow{12}{*}{\textbf{MNIST}}}      & \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{MVI}}} & \textbf{MEAN}    & 4.3180          & 0.5686          & 0.6716          & 6.1985          & 0.5144          & 0.6420          & 1.0775          & 0.5723          & 0.6753          \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              & \textbf{LR}      & 1.7631          & 0.5681          & 0.7393          & 1.4520          & 0.5107          & 0.6836          & 1.1607          & 0.5710          & 0.6734          \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              & \textbf{GR}      & 1.6997          & 0.5684          & 0.7574          & 1.5506          & 0.5718          & 0.6846          & 1.2489          & 0.5796          & 0.6732          \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              & \textbf{KFMC}    & 1.1844          & 0.5682          & 0.7520          & 1.0467          & 0.5711          & 0.6846          & 1.5782          & 0.5804          & 0.6744          \\ \cline{2-12} 
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{MF}}}  & \textbf{FGSR}    & 1.1400          & 0.5956          & 0.7262          & 1.7700          & 0.5956          & 0.6262          & 1.0010          & 0.5956          & 0.6262          \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              & \textbf{BPMF}    & 0.8578          & 0.5956          & 0.7262          & 1.4304          & 0.5956          & 0.6262          & 0.9318          & 0.5956          & 0.6262          \\ \cline{2-12} 
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{PSD}}} & \textbf{CMC}     & 0.9375          & 0.5824          & 0.7885          & 0.9515          & 0.5838          & 0.6852          & 0.6841          & 0.5787          & 0.5844          \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              & \textbf{DMC}     & 0.7385          & 0.5778          & 0.7653          & 0.8565          & 0.5838          & 0.6854          & 0.6632          & 0.5787          & 0.5863          \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              &  \textbf{FMC}\cite{ma2024fast}     & 0.7231          & 0.5785          & 0.6965          & 0.8480          & 0.6180          & 0.6697          & 0.6618          & \textbf{0.6774} & 0.7196          \\ \cline{2-12} 
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{LR}}}  & \textbf{NNFN}    & 0.7025          & 0.5763          & 0.7623          & 0.8963          & 0.5822          & 0.6866          & 0.7007          & 0.5796          & 0.5865          \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              & \textbf{facNNFN} & 1.4114          & 0.5722          & 0.7852          & 1.0728          & 0.5711          & 0.6912          & 1.2450          & 0.5686          & 0.5877          \\ \hline
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{OUR}}} & \textbf{SSNN}    & \textbf{0.6509} & \textbf{0.6400} & \textbf{0.7889} & \textbf{0.8312} & \textbf{0.6330} & \textbf{0.6981} & \textbf{0.6521} & \textbf{0.6350} & \textbf{0.7512} \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              & \textbf{SSNmF}   & \textbf{0.6584} & \textbf{0.6317} & \textbf{0.7851} & \textbf{0.8231} & \textbf{0.6233} & \textbf{0.6981} & \textbf{0.6597} & 0.6348          & \textbf{0.7175} \\ \hline
\multicolumn{1}{c|}{\multirow{12}{*}{\textbf{PROTEIN}}}    & \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{MVI}}} & \textbf{MEAN}    & 3.2905          & 0.5811          & 0.6859          & 4.1765          & 0.6791          & 0.6850          & 5.0652          & 0.5700          & 0.7354          \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              & \textbf{LR}      & 2.6848          & 0.5392          & 0.6916          & 3.4045          & 0.6736          & 0.6807          & 3.1311          & 0.6271          & 0.7087          \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              & \textbf{GR}      & 2.6753          & 0.5801          & 0.6940          & 1.5771          & 0.6753          & 0.6825          & 2.2553          & 0.7206          & 0.7075          \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              & \textbf{KFMC}    & 1.0109          & 0.5606          & 0.6933          & 1.8972          & 0.6738          & 0.6822          & 1.5423          & 0.7263          & 0.7178          \\ \cline{2-12} 
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{MF}}}  & \textbf{FGSR}    & 1.1800          & 0.4969          & 0.6232          & 1.1710          & 0.5969          & 0.7232          & 1.1380          & 0.6969          & 0.7023          \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              & \textbf{BPMF}    & 0.7658          & 0.5969          & 0.6232          & 0.7990          & 0.6969          & 0.7232          & 1.1082          & 0.6969          & 0.7023          \\ \cline{2-12} 
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{PSD}}} & \textbf{CMC}     & 0.7477          & 0.5931          & 0.6540          & 0.7888          & 0.6906          & 0.7284          & 0.7166          & 0.6883          & 0.7412          \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              & \textbf{DMC}     & 0.8308          & 0.6131          & 0.6976          & 0.7807          & 0.6913          & 0.7285          & 0.7150          & 0.6882          & 0.7541          \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              &  \textbf{FMC}\cite{ma2024fast}     & 0.7145          & 0.6197          & 0.6997          & 0.8116          & 0.6935          & 0.6997          & 0.7347          & 0.6688          & 0.6958          \\ \cline{2-12} 
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{LR}}}  & \textbf{NNFN}    & 0.8532          & 0.6130          & 0.6924          & 0.7909          & 0.7134          & 0.7386          & 0.8553          & 0.6801          & \textbf{0.7630} \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              & \textbf{facNNFN} & 0.9242          & 0.6211          & 0.6953          & 0.7930          & 0.7107          & 0.7389          & 0.9589          & 0.7212          & \textbf{0.7764} \\ \hline
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{OUR}}} & \textbf{SSNN}    & \textbf{0.7096} & \textbf{0.6467} & \textbf{0.7197} & \textbf{0.7083} & \textbf{0.7363} & \textbf{0.7493} & \textbf{0.6729} & \textbf{0.7352} & 0.7516          \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              & \textbf{SSNmF}   & \textbf{0.7029} & \textbf{0.6471} & \textbf{0.7181} & \textbf{0.7082} & \textbf{0.7346} & \textbf{0.7551} & \textbf{0.6791} & \textbf{0.7354} & 0.7216          \\ \hline
\multicolumn{1}{c|}{\multirow{12}{*}{\textbf{CIFAR10}}}    & \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{MVI}}} & \textbf{MEAN}    & 1.3288          & 0.6542          & 0.7839          & 5.3787          & 0.6230          & 0.6791          & 1.1631          & 0.6205          & 0.7462          \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              & \textbf{LR}      & 1.5060          & 0.6833          & 0.7810          & 2.4600          & 0.6314          & 0.6773          & 2.3465          & 0.5829          & 0.7870          \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              & \textbf{GR}      & 1.4112          & 0.6429          & 0.7864          & 3.8330          & 0.6130          & 0.6798          & 1.5646          & 0.6396          & 0.7882          \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              & \textbf{KFMC}    & 1.9599          & 0.6852          & 0.7946          & 2.1048          & 0.6011          & 0.6791          & 1.5563          & 0.6067          & 0.7867          \\ \cline{2-12} 
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{MF}}}  & \textbf{BPMF}    & 1.6420          & 0.6101          & 0.7417          & 2.0260          & 0.6013          & 0.6742          & 3.7330          & 0.6101          & 0.7942          \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              & \textbf{FGSR}    & 1.1000          & 0.6265          & 0.7969          & 1.7000          & 0.6530          & 0.6797          & 1.0330          & 0.6053          & 0.7969          \\ \cline{2-12} 
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{PSD}}} & \textbf{CMC}     & 0.8864          & 0.6288          & 0.7540          & 0.7510          & 0.6350          & 0.6854          & 0.5720          & 0.6081          & 0.7854          \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              & \textbf{DMC}     & 0.8323          & 0.6288          & 0.7643          & 0.7352          & 0.6538          & 0.6865          & 0.5956          & 0.6078          & 0.7863          \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              &  \textbf{FMC}\cite{ma2024fast}     & 0.8145          & 0.6303          & 0.7907          & 0.8116          & 0.6333          & 0.6400          & 0.5648          & 0.6134          & 0.7565          \\ \cline{2-12} 
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{LR}}}  & \textbf{NNFN}    & 0.7388          & \textbf{0.6806} & 0.7430          & 0.7308          & 0.6172          & 0.6854          & 0.5930          & 0.6088          & 0.7865          \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              & \textbf{facNNFN} & 1.3090          & 0.6211          & 0.7430          & 0.8360          & 0.6112          & 0.6914          & 0.8173          & 0.6012          & 0.7842          \\ \hline
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{OUR}}} & \textbf{SSNN}    & \textbf{0.7137} & \textbf{0.6458} & \textbf{0.7950} & \textbf{0.7174} & \textbf{0.6625} & \textbf{0.6929} & \textbf{0.5610} & \textbf{0.6208} & \textbf{0.7949} \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                              & \textbf{SSNmF}   & \textbf{0.7138} & 0.6454          & \textbf{0.7910} & \textbf{0.7080} & \textbf{0.6610} & \textbf{0.6525} & \textbf{0.5365} & \textbf{0.6238} & \textbf{0.7941} \\ \hline
\bottomrule
\end{tabular} 
}
\end{table*}

==> Table/Ablation/Q2S4.tex <==
\begin{table*}[!htb]
\centering
\scriptsize 
\caption{Ablation study on various variations of RMSE, Recall@top20\%, nDCG@top20\% with $m=4,000$ search candidates and $n=200$ query items, where missing ratio $\rho =\{0.7,0.8,0.9\}$, rank $r = 100$, $\lambda = 0.001$, $\gamma = 0.001$, and $T = 10,000$. The top 2 performances are highlighted in bold.} 
\label{tab:ab:Q2S4} 
\resizebox{0.9\columnwidth}{!}{ 
\begin{tabular}{ll|lll|lll|lll}
\toprule
\hline
\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Dataset/Method}}}                      & \multicolumn{3}{c|}{\textbf{0.7}}                   & \multicolumn{3}{c|}{\textbf{0.8}}                   & \multicolumn{3}{c}{\textbf{0.9}}                    \\   \cline{3-11} 
\multicolumn{2}{c|}{}          & \textbf{RMSE}   & \textbf{Recall} & \textbf{nDCG}   & \textbf{RMSE}   & \textbf{Recall} & \textbf{nDCG}   & \textbf{RMSE}   & \textbf{Recall} & \textbf{nDCG}   \\ \hline
\multicolumn{1}{l|}{\multirow{13}{*}{\textbf{ImageNet}}}  & \textbf{SMC\_F}& 0.9995          & 0.5153          & 0.6535          & 0.7391          & 0.5146          & 0.6659          & 0.7890          & 0.6724          & 0.7164          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_NR}& 0.9993          & 0.5311          & 0.6424          & 0.7389          & 0.5537          & 0.6659          & 0.7846          & 0.6774          & 0.7176          \\ 
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_GD} & 0.6500 & 0.6000 & 0.7135 & 0.6745 & 0.6345 & 0.6710 & 0.5896 & 0.7016 & 0.7606 \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_QN}& 1.1249          & 0.5315          & 0.6643          & 0.7019          & 0.5336          & 0.6655          & 0.7840          & 0.5979          & 0.7176          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNN\_QN}& 1.1170          & 0.5249          & 0.6633          & 0.7024          & 0.5457          & 0.6655          & 0.7851          & 0.5868          & 0.7014          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNmF\_QN}& 1.1162          & 0.5135          & 0.6634          & 0.7024          & 0.5436          & 0.6646          & 0.7130          & 0.5859          & 0.7032          \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{MC\_ON} & 0.7330          & 0.5435          & 0.6643          & 1.0010          & 0.4965          & 0.6341          & 0.7679          & 0.5894          & 0.7056          \\
\multicolumn{1}{l|}{}                                     & \textbf{MC\_fON} & 0.7162          & 0.5449          & 0.6643          & 1.0012          & 0.4964          & 0.6341          & 0.7863          & 0.5894          & 0.7054          \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{CMC} \cite{li2015estimating}       & 0.6915          & 0.5715          & 0.6713          & 0.7270          & 0.5610          & 0.6834          & 0.6494          & 0.6148          & \textbf{0.7416} \\
\multicolumn{1}{l|}{}                                     & \textbf{DMC} \cite{li2020scalable}     & 0.6906          & 0.5752          & 0.6709          & 0.7249          & 0.5749          & 0.6865          & 0.6017          & 0.6312          & 0.7683          \\
\multicolumn{1}{c|}{}                                     &  \textbf{FMC}\cite{ma2024fast}    & 0.7491                     & 0.6398                     & 0.7565                     & 0.6731                     & 0.6576                     & 0.7488                     & 0.5999 & 0.6157 & 0.7910 \\  \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{SMCNN (OURS)}     & \textbf{0.6105} & \textbf{0.6323} & \textbf{0.7177} & \textbf{0.5983} & \textbf{0.6000} & \textbf{0.6956} & \textbf{0.5634} & \textbf{0.7036} & \textbf{0.7929} \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNmF (OURS)}    & \textbf{0.6063} & \textbf{0.6296} & \textbf{0.7047} & \textbf{0.5967} & \textbf{0.6042} & \textbf{0.6956} & \textbf{0.5730} & \textbf{0.7080} & \textbf{0.7443} \\  \hline
\multicolumn{1}{l|}{\multirow{13}{*}{\textbf{MNIST}}}     & \textbf{SMC\_F}& 1.1872          & 0.6765          & 0.6628          & 0.7760          & 0.6537          & 0.6821          & 0.8409          & 0.5862          & 0.7666          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_NR}& 1.1872          & 0.6858          & 0.6628          & 0.7670          & 0.6472          & 0.6820          & 0.8409          & 0.5861          & 0.7686          \\ 
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_GD} & 0.7960 & 0.7050 & 0.7993 & 0.6493 & 0.6156 & 0.7650 & 0.6490 & 0.6445 & 0.8645 \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_QN}& 1.1507          & 0.6765          & 0.6616          & 0.7762          & 0.6243          & 0.6805          & 0.8326          & 0.5760          & 0.7861          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNN\_QN}& 1.1510          & 0.6877          & 0.6616          & 0.7762          & 0.6225          & 0.6805          & 0.8328          & 0.5860          & 0.7546          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNmF\_QN}& 1.1510          & 0.6556          & 0.6616          & 0.7625          & 0.6235          & 0.6805          & 0.8328          & 0.5860          & 0.7681          \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{MC\_ON} & 0.8978          & 0.7157          & 0.6616          & 0.7655          & 0.6154          & 0.6616          & 0.8321          & 0.6042          & 0.7686          \\
\multicolumn{1}{l|}{}                                     & \textbf{MC\_fON} & 0.8678          & 0.7177          & 0.6616          & 0.7510          & 0.6352          & 0.6616          & 0.8123          & 0.6115          & 0.7892          \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{CMC} \cite{li2015estimating}       & 0.8563          & 0.6725          & 0.7820          & 0.8680          & 0.6278          & 0.7642          & 0.6510          & 0.6068          & 0.8134          \\
\multicolumn{1}{l|}{}                                     & \textbf{DMC} \cite{li2020scalable}     & 0.8012          & 0.6735          & 0.7636          & 0.7162          & 0.6195          & 0.7410          & 0.6718          & 0.6130          & 0.8510          \\
\multicolumn{1}{c|}{}                                     &  \textbf{FMC}\cite{ma2024fast}    & 0.6559                     & 0.6278                     & 0.6965                     & 0.6509                     & 0.6005                     & 0.6540                     & 0.5943 & 0.7193 & 0.7200 \\  \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{SMCNN (OURS)}     & \textbf{0.7843} & \textbf{0.7363} & \textbf{0.8193} & \textbf{0.6260} & \textbf{0.6460} & \textbf{0.7844} & \textbf{0.6425} & \textbf{0.6533} & \textbf{0.8948} \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNmF (OURS)}    & \textbf{0.7328} & \textbf{0.7288} & \textbf{0.8033} & \textbf{0.6518} & \textbf{0.6708} & \textbf{0.7869} & \textbf{0.6415} & \textbf{0.6500} & \textbf{0.8931} \\  \hline
\multicolumn{1}{l|}{\multirow{13}{*}{\textbf{PROTEIN}}}   & \textbf{SMC\_F}& 0.9103          & 0.6135          & 0.6863          & 0.7745          & 0.6465          & 0.7040          & 0.8022          & 0.6436          & 0.7866          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_NR}& 0.9225          & 0.6415          & 0.6964          & 0.7754          & 0.6455          & 0.7097          & 0.8022          & 0.6436          & 0.7830          \\ 
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_GD} & 0.7670 & 0.7170 & 0.7083 & 0.6883 & 0.6084 & 0.7857 & 0.5921 & 0.7008 & 0.8084 \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_QN}& 0.9181          & 0.6155          & 0.6944          & 0.7754          & 0.6456          & 0.7011          & 0.8007          & 0.6544          & 0.7870          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNN\_QN}& 0.9179          & 0.6450          & 0.6931          & 0.7653          & 0.6457          & 0.7131          & 0.8009          & 0.6544          & 0.7803          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNmF\_QN}& 0.9179          & 0.6155          & 0.6934          & 0.7653          & 0.6457          & 0.7138          & 0.8008          & 0.6538          & 0.7860          \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{MC\_ON} & 0.9213          & 0.6432          & 0.6934          & 0.7432          & 0.6772          & 0.7116          & 0.7012          & 0.6715          & 0.7866          \\
\multicolumn{1}{l|}{}                                     & \textbf{MC\_fON} & 0.9410          & 0.6772          & 0.6943          & 0.7515          & 0.6572          & 0.7217          & 0.7901          & 0.6715          & 0.7666          \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{CMC} \cite{li2015estimating}       & 0.8477          & 0.6931          & 0.7814          & 0.7888          & 0.6062          & 0.7851          & 0.6585          & 0.6887          & 0.8234          \\
\multicolumn{1}{l|}{}                                     & \textbf{DMC} \cite{li2020scalable}     & 0.8308          & 0.6931          & 0.7843          & 0.7807          & 0.6130          & 0.7522          & 0.6497          & 0.6886          & 0.8334          \\
\multicolumn{1}{c|}{}                                      &  \textbf{FMC}\cite{ma2024fast}  & 0.7627                     & 0.7274                     & 0.7965                     & 0.7316                     & 0.6774                     & 0.6997                     & 0.6506 & 0.6289 & 0.8920 \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{SMCNN (OURS)}     & \textbf{0.7506} & \textbf{0.7183} & \textbf{0.7917} & \textbf{0.6574} & \textbf{0.6313} & \textbf{0.7934} & \textbf{0.5390} & \textbf{0.7323} & \textbf{0.8477} \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNmF (OURS)}    & \textbf{0.7526} & \textbf{0.7198} & \textbf{0.7913} & \textbf{0.6446} & \textbf{0.6333} & \textbf{0.7914} & \textbf{0.5828} & \textbf{0.7080} & \textbf{0.8413} \\  \hline
\multicolumn{1}{l|}{\multirow{13}{*}{\textbf{CIFAR}}}     & \textbf{SMC\_F}& 0.8718          & 0.6514          & 0.6566          & 0.7342          & 0.6454          & 0.6194          & 0.8071          & 0.6987          & 0.6855          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_NR}& 0.8718          & 0.6545          & 0.6758          & 0.7342          & 0.6742          & 0.6194          & 0.8070          & 0.6786          & 0.6756          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_GD} & 0.7686 & 0.7080 & 0.8139 & 0.7239 & 0.6239 & 0.7695 & 0.6559 & 0.7057 & 0.8057 \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_QN}& 0.8737          & 0.6572          & 0.6546          & 0.7812          & 0.6744          & 0.6239          & 0.8057          & 0.6885          & 0.6786          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNN\_QN}& 0.8723          & 0.6739          & 0.6281          & 0.7823          & 0.6744          & 0.6239          & 0.8058          & 0.6866          & 0.6866          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNmF\_QN}& 0.8730          & 0.6798          & 0.6758          & 0.7842          & 0.6736          & 0.6239          & 0.8058          & 0.6989          & 0.6756          \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{MC\_ON} & 0.7914          & 0.6765          & 0.6565          & 0.7880          & 0.6772          & 0.6616          & 0.7844          & 0.7154          & 0.6676          \\
\multicolumn{1}{l|}{}                                     & \textbf{MC\_fON} & 0.7950          & 0.6857          & 0.6676          & 0.7689          & 0.6572          & 0.6616          & 0.7893          & 0.7154          & 0.6477          \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{CMC} \cite{li2015estimating}       & 0.7939          & 0.7113          & 0.7140          & 0.7648          & 0.6728          & 0.6831          & 0.7136          & 0.6803          & 0.7825          \\
\multicolumn{1}{l|}{}                                     & \textbf{DMC} \cite{li2020scalable}     & 0.7931          & 0.7135          & 0.7520          & 0.7628          & 0.6715          & 0.6841          & 0.7292          & 0.6800          & 0.7409          \\
\multicolumn{1}{c|}{}                                      &  \textbf{FMC}\cite{ma2024fast}    & 0.7559                     & 0.7054                     & 0.7942                     & 0.6565                     & 0.6181                     & 0.7988                     & 0.6249 & 0.7009 & 0.7819 \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{SMCNN (OURS)}     & \textbf{0.7527} & \textbf{0.7234} & \textbf{0.8947} & \textbf{0.7189} & \textbf{0.6318} & \textbf{0.7942} & \textbf{0.6486} & \textbf{0.7204} & \textbf{0.8310} \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNmF (OURS)}    & \textbf{0.7506} & \textbf{0.7146} & \textbf{0.8948} & \textbf{0.7179} & \textbf{0.6295} & \textbf{0.7795} & \textbf{0.6493} & \textbf{0.7267} & \textbf{0.8310} \\  \hline
\multicolumn{1}{l|}{\multirow{13}{*}{\textbf{GoogleNews}}} & \textbf{SMC\_F}& 0.8279          & 0.6021          & 0.6494          & 0.7274          & 0.5866          & 0.6931          & 0.6427          & 0.5471          & 0.7765          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_NR}& 0.8280          & 0.6321          & 0.6434          & 0.7275          & 0.5783          & 0.6931          & 0.6471          & 0.5668          & 0.7562          \\ 
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_GD} & 0.7457 & 0.6550 & 0.7220 & 0.6720 & 0.6820 & 0.8078 & 0.6137 & 0.6358 & 0.8058\\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_QN}& 0.8797          & 0.6090          & 0.6940          & 0.7454          & 0.5766          & 0.6793          & 0.6537          & 0.5833          & 0.7652          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNN\_QN}& 0.8797          & 0.6029          & 0.6440          & 0.7454          & 0.5676          & 0.6793          & 0.6137          & 0.5483          & 0.7652          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNmF\_QN}& 0.8796          & 0.6229          & 0.6840          & 0.7457          & 0.5667          & 0.6793          & 0.6235          & 0.4833          & 0.7231          \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{MC\_ON} & 0.8150          & 0.6000          & 0.6869          & 0.7180          & 0.5642          & 0.6876          & 0.6554          & 0.5979          & 0.7843          \\
\multicolumn{1}{l|}{}                                     & \textbf{MC\_fON} & 0.9449          & 0.6135          & 0.6936          & 0.6834          & 0.5188          & 0.6927          & 0.6761          & 0.5583          & 0.6817          \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{CMC} \cite{li2015estimating}       & 0.7718          & 0.6202          & 0.7841          & 0.6944          & 0.5680          & 0.7560          & 0.6667          & 0.5739          & 0.7340          \\
\multicolumn{1}{l|}{}                                     & \textbf{DMC} \cite{li2020scalable}     & 0.7823          & 0.6262          & 0.7853          & 0.7131          & 0.5680          & 0.7533          & 0.6551          & 0.5717          & 0.7230          \\
\multicolumn{1}{c|}{}                                     &  \textbf{FMC}\cite{ma2024fast}    &  0.7573  & 0.7114  &  0.7944  & 0.7664 &0.6715  &  0.7883 & 0.6711 & 0.7083 & 0.7997 \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{SMCNN (OURS)}     & \textbf{0.7233} & \textbf{0.6438} & \textbf{0.7749} & \textbf{0.6543} & \textbf{0.6708} & \textbf{0.7966} & \textbf{0.5970} & \textbf{0.6398} & \textbf{0.8242} \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNmF (OURS)}    & \textbf{0.7134} & \textbf{0.6438} & \textbf{0.7749} & \textbf{0.6534} & \textbf{0.6708} & \textbf{0.7966} & \textbf{0.5979} & \textbf{0.6408} & \textbf{0.8082}\\
\hline
\bottomrule
\end{tabular} 
}
\end{table*}

==> Table/Ablation/Q2S5.tex <==
\begin{table*}[!htb]
\centering
\scriptsize 
\caption{Ablation study on various variations of RMSE, Recall@top20\%, nDCG@top20\% with $m=5,000$ search candidates and $n=200$ query items, where missing ratio $\rho =\{0.7,0.8,0.9\}$, rank $r = 100$, $\lambda = 0.001$, $\gamma = 0.001$, and $T = 10,000$. The top 2 performances are highlighted in bold.} 
\label{tab:ab:Q2S5} 
\resizebox{0.9\columnwidth}{!}{ 
\begin{tabular}{ll|lll|lll|lll}
\toprule
\hline
\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Dataset/Method}}}                      & \multicolumn{3}{c|}{\textbf{0.7}}                   & \multicolumn{3}{c|}{\textbf{0.8}}                   & \multicolumn{3}{c}{\textbf{0.9}}                    \\   \cline{3-11} 
\multicolumn{2}{c|}{}          & \textbf{RMSE}   & \textbf{Recall} & \textbf{nDCG}   & \textbf{RMSE}   & \textbf{Recall} & \textbf{nDCG}   & \textbf{RMSE}   & \textbf{Recall} & \textbf{nDCG}   \\ \hline
\multicolumn{1}{l|}{\multirow{13}{*}{\textbf{ImageNet}}}  & \textbf{SMC\_F} & 0.7437          & 0.7134          & 0.7942          & 0.9490          & 0.4187          & 0.6666          & 0.8531          & 0.6433          & 0.6867          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_NR} & 0.7439          & 0.7132          & 0.7952          & 0.9487          & 0.4173          & 0.6666          & 0.8531          & 0.6235          & 0.6874          \\ 
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_GD} & 0.7611 & 0.7400 & 0.8973 & 0.6173 & 0.6413 & 0.7870 & 0.5830 & 0.6323 & 0.7323 \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_QN} & 0.7130          & 0.7142          & 0.8146          & 1.0206          & 0.4133          & 0.6667          & 0.8611          & 0.6445          & 0.6774          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNN\_QN} & 0.7420          & 0.7145          & 0.8432          & 1.0210          & 0.4133          & 0.6667          & 0.8593          & 0.6155          & 0.6867          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNmF\_QN} & 0.7243          & 0.7153          & 0.8432          & 1.0209          & 0.4133          & 0.6667          & 0.8593          & 0.6135          & 0.6542          \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{MC\_ON} & 0.7534          & 0.7152          & 0.8516          & 0.7053          & 0.4587          & 0.7016          & 0.7053          & 0.6319          & 0.6435          \\
\multicolumn{1}{l|}{}                                     & \textbf{MC\_fON} & 0.7343          & 0.7146          & 0.8634          & 0.7053          & 0.4587          & 0.7016          & 0.7053          & 0.6139          & 0.6716          \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{CMC} \cite{li2015estimating}    & 0.7504          & 0.7347          & 0.8342          & 0.6355          & 0.5691          & 0.7841          & 0.5670          & 0.6317          & 0.6988          \\
\multicolumn{1}{l|}{}                                     & \textbf{DMC} \cite{li2020scalable}    & 0.7358          & 0.7335          & 0.9042          & 0.6375          & 0.5693          & 0.7854          & 0.5344          & 0.6331          & 0.7011          \\
\multicolumn{1}{c|}{}                                      &  \textbf{FMC}\cite{ma2024fast}    &  0.7278                     & 0.7680                     & 0.7398                     & 0.6934                     & 0.6932                     & 0.7997                     & 0.7158 & 0.6185 & 0.7949 \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{SMCNN (OURS)}     & \textbf{0.7110} & \textbf{0.7433} & \textbf{0.9070} & \textbf{0.6187} & \textbf{0.6446} & \textbf{0.7986} & \textbf{0.5128} & \textbf{0.6625} & \textbf{0.7896} \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNmF (OURS)}    & \textbf{0.7104} & \textbf{0.7363} & \textbf{0.9065} & \textbf{0.6238} & \textbf{0.6429} & \textbf{0.7984} & \textbf{0.5127} & \textbf{0.6620} & \textbf{0.7897} \\  \hline
\multicolumn{1}{l|}{\multirow{13}{*}{\textbf{MNIST}}}     & \textbf{SMC\_F} & 0.7902          & 0.8014          & 0.8757          & 0.6690          & 0.6960          & 0.6915          & 0.7433          & 0.6547          & 0.7704          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_NR} & 0.7902          & 0.8032          & 0.8648          & 0.6690          & 0.6960          & 0.6915          & 0.7434          & 0.6547          & 0.7860          \\ 
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_GD} & 0.7360 & 0.8520 & 0.8784 & 0.6384 & 0.8194 & 0.8460 & 0.6190 & 0.7269 & 0.8269 \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_QN} & 0.7834          & 0.8135          & 0.8683          & 0.6694          & 0.6827          & 0.6919          & 0.7435          & 0.6455          & 0.7798          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNN\_QN} & 0.7839          & 0.8325          & 0.8630          & 0.6698          & 0.6827          & 0.6919          & 0.7437          & 0.6654          & 0.7870          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNmF\_QN} & 0.7839          & 0.8232          & 0.8930          & 0.6698          & 0.6827          & 0.6919          & 0.7437          & 0.6654          & 0.7977          \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{MC\_ON} & 0.7973          & 0.8137          & 0.8650          & 0.7053          & 0.5459          & 0.7016          & 0.7452          & 0.6539          & 0.7016          \\
\multicolumn{1}{l|}{}                                     & \textbf{MC\_fON} & 0.7898          & 0.8326          & 0.8650          & 0.7053          & 0.5459          & 0.7016          & 0.7455          & 0.6537          & 0.8132          \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{CMC} \cite{li2015estimating}    & 0.8326          & 0.8410          & 0.8451          & 0.6575          & 0.8170          & 0.7854          & 0.5769          & 0.7548          & 0.8431          \\
\multicolumn{1}{l|}{}                                     & \textbf{DMC} \cite{li2020scalable}    & 0.7634          & 0.8424          & 0.8544          & 0.6705          & 0.8198          & 0.7859          & 0.5954          & 0.7408          & 0.8534          \\
\multicolumn{1}{c|}{}                                      &  \textbf{FMC}\cite{ma2024fast}    & 0.7682                     & 0.7315                     & 0.8748                     & 0.6582                     & 0.6392                     & 0.7680                     & 0.5589 & 0.6780 & 0.6997 \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{SMCNN (OURS)}     & \textbf{0.7197} & \textbf{0.8688} & \textbf{0.8969} & \textbf{0.6237} & \textbf{0.8021} & \textbf{0.8370} & \textbf{0.5653} & \textbf{0.7696} & \textbf{0.8580} \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNmF (OURS)}    & \textbf{0.7128} & \textbf{0.8563} & \textbf{0.8973} & \textbf{0.6233} & \textbf{0.8208} & \textbf{0.8364} & \textbf{0.5438} & \textbf{0.7460} & \textbf{0.8640} \\  \hline
\multicolumn{1}{l|}{\multirow{13}{*}{\textbf{PROTEIN}}}   & \textbf{SMC\_F} & 0.7212          & 0.6114          & 0.8414          & 0.7241          & 0.5333          & 0.6352          & 0.7487          & 0.5943          & 0.7040          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_NR} & 0.7432          & 0.6036          & 0.8134          & 0.7241          & 0.5320          & 0.6350          & 0.7486          & 0.5925          & 0.7040          \\ 
\multicolumn{1}{l|}{}                                      & \textbf{SMC\_GD} & 0.6940 & 0.6830 & 0.8481 & 0.6841 & 0.6481 & 0.8470 & 0.8314 & 0.6216 & 0.8016 \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_QN} & 0.7144          & 0.6127          & 0.8244          & 0.7352          & 0.5293          & 0.6358          & 0.7455          & 0.5635          & 0.7042          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNN\_QN} & 0.7123          & 0.6134          & 0.8244          & 0.7352          & 0.5293          & 0.6357          & 0.7457          & 0.5658          & 0.7042          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNmF\_QN} & 0.7314          & 0.6304          & 0.8454          & 0.7350          & 0.5293          & 0.6358          & 0.7456          & 0.5635          & 0.7042          \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{MC\_N} & 0.7135          & 0.6187          & 0.8170          & 0.7413          & 0.5587          & 0.7016          & 0.7443          & 0.5845          & 0.7016          \\
\multicolumn{1}{l|}{}                                     & \textbf{MC\_fON} & 0.7315          & 0.6144          & 0.8135          & 0.7995          & 0.5587          & 0.7016          & 0.7423          & 0.5924          & 0.7016          \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{CMC} \cite{li2015estimating}    & 0.7314          & 0.6575          & 0.8445          & 0.6974          & 0.6414          & 0.8320          & 0.7783          & 0.6153          & 0.7031          \\
\multicolumn{1}{l|}{}                                     & \textbf{DMC} \cite{li2020scalable}    & 0.7351          & 0.6582          & 0.8650          & 0.6794          & 0.6351          & 0.7913          & 0.7653          & 0.6148          & 0.6994          \\
\multicolumn{1}{c|}{}                                      &  \textbf{FMC}\cite{ma2024fast}    &  0.7358                     & 0.8306                     & 0.8974                     & 0.6355                     & 0.7919                     & 0.8268                     & 0.5623 & 0.7278 & 0.7997 \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{SMCNN (OURS)}     & \textbf{0.6508} & \textbf{0.6896} & \textbf{0.8755} & \textbf{0.6240} & \textbf{0.6104} & \textbf{0.8699} & \textbf{0.5735} & \textbf{0.6688} & \textbf{0.8858} \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNmF (OURS)}    & \textbf{0.6442} & \textbf{0.6904} & \textbf{0.8663} & \textbf{0.6402} & \textbf{0.6167} & \textbf{0.8566} & \textbf{0.5900} & \textbf{0.6521} & \textbf{0.8838} \\  \hline
\multicolumn{1}{l|}{\multirow{13}{*}{\textbf{CIFAR}}}     & \textbf{SMC\_F} & 0.7659          & 0.5184          & 0.6865          & 0.8584          & 0.5445          & 0.6000          & 0.7177          & 0.5365          & 0.6878          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_NR} & 0.7650          & 0.5318          & 0.6675          & 0.8584          & 0.5445          & 0.6000          & 0.7176          & 0.5337          & 0.6887          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_GD} & 0.6530 & 0.6560 & 0.8333 & 0.6383 & 0.6912 & 0.6918 & 0.5843 & 0.6434 & 0.7434 \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_QN} & 0.7653          & 0.5319          & 0.6865          & 0.8584          & 0.5451          & 0.6014          & 0.7162          & 0.5134          & 0.6977          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNN\_QN} & 0.7469          & 0.5319          & 0.6358          & 0.8584          & 0.5451          & 0.6014          & 0.7163          & 0.5124          & 0.6977          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNmF\_QN} & 0.7693          & 0.5315          & 0.6736          & 0.8584          & 0.5451          & 0.6014          & 0.7163          & 0.5126          & 0.6976          \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{MC\_ON} & 0.7765          & 0.5139          & 0.6888          & 0.8143          & 0.5459          & 0.7016          & 0.7415          & 0.5252          & 0.7016          \\
\multicolumn{1}{l|}{}                                     & \textbf{MC\_fON} & 0.7547          & 0.5246          & 0.6877          & 0.8053          & 0.5459          & 0.7016          & 0.7341          & 0.5249          & 0.7016          \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{CMC} \cite{li2015estimating}    & 0.8773          & 0.5810          & 0.7855          & 0.8373          & 0.6192          & 0.6530          & 0.6735          & 0.5612          & 0.6735          \\
\multicolumn{1}{l|}{}                                     & \textbf{DMC} \cite{li2020scalable}    & 0.8256          & 0.5802          & 0.7835          & 0.8121          & 0.6263          & 0.6530          & 0.5822          & 0.5672          & 0.6784          \\
\multicolumn{1}{c|}{}                                      &  \textbf{FMC}\cite{ma2024fast}    & 0.6865                     & 0.6701                     & 0.7997                     & 0.6200                     & 0.6116                     & 0.7971                     & 0.6145 & 0.6475 & 0.7703 \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{SMCNN (OURS)}     & \textbf{0.6868} & \textbf{0.6446} & \textbf{0.8555} & \textbf{0.5942} & \textbf{0.6960} & \textbf{0.6934} & \textbf{0.5213} & \textbf{0.6563} & \textbf{0.7975} \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNmF (OURS)}    & \textbf{0.6379} & \textbf{0.6429} & \textbf{0.8387} & \textbf{0.5841} & \textbf{0.6938} & \textbf{0.6941} & \textbf{0.5289} & \textbf{0.6583} & \textbf{0.7972} \\ \hline
\multicolumn{1}{l|}{\multirow{13}{*}{\textbf{GoogleNews}}} & \textbf{SMC\_F} & 0.8411          & 0.6823          & 0.6995          & 0.7115          & 0.6255          & 0.7563          & 0.7540          & 0.5648          & 0.6769          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_NR} & 0.8431          & 0.6844          & 0.6795          & 0.7141          & 0.6546          & 0.7977          & 0.7441          & 0.5665          & 0.6790          \\ 
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_GD} & 0.7431 & 0.7540 & 0.7346 & 0.6946 & 0.6346 & 0.7486 & 0.7217 & 0.6262 & 0.7842 \\\cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{SMC\_QN} & 0.7514          & 0.6819          & 0.6459          & 0.7041          & 0.6546          & 0.7766          & 0.7452          & 0.5673          & 0.6790          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNN\_QN} & 0.7557          & 0.6569          & 0.6995          & 0.7061          & 0.6456          & 0.7683          & 0.7420          & 0.5673          & 0.6790          \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNmF\_QN} & 0.7965          & 0.6976          & 0.6947          & 0.7316          & 0.6646          & 0.7893          & 0.7562          & 0.5647          & 0.6790          \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{MC\_ON} & 0.7110          & 0.6831          & 0.7082          & 0.6930          & 0.6131          & 0.7541          & 0.7620          & 0.5674          & 0.6710          \\
\multicolumn{1}{l|}{}                                     & \textbf{MC\_fON} & 0.6515          & 0.6850          & 0.6944          & 0.6275          & 0.5542          & 0.7926          & 0.7199          & 0.5655          & 0.6789          \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{CMC} \cite{li2015estimating}    & 0.8996          & 0.7014          & 0.7134          & 0.8331          & 0.6817          & 0.8019          & 0.7165          & 0.5150          & 0.7040          \\
\multicolumn{1}{l|}{}                                     & \textbf{DMC} \cite{li2020scalable}    & 0.8849          & 0.7155          & 0.7290          & 0.7187          & 0.6879          & 0.8342          & 0.7536          & 0.6151          & 0.7020          \\
\multicolumn{1}{c|}{}                                      &  \textbf{FMC}\cite{ma2024fast}    &   0.6977 &  0.6486 &  0.7997  &  0.5975  &  0.6621  &  0.6972 & 0.5448 & 0.6028 & 0.7970 \\ \cline{2-11}
\multicolumn{1}{l|}{}                                     & \textbf{SMCNN (OURS)}     & \textbf{0.7278} & \textbf{0.7625} & \textbf{0.7493} & \textbf{0.6813} & \textbf{0.6980} & \textbf{0.8188} & \textbf{0.7031} & \textbf{0.6421} & \textbf{0.8172} \\
\multicolumn{1}{l|}{}                                     & \textbf{SMCNmF (OURS)}    & \textbf{0.7241} & \textbf{0.7625} & \textbf{0.7314} & \textbf{0.6960} & \textbf{0.6988} & \textbf{0.8050} & \textbf{0.7041} & \textbf{0.6421} & \textbf{0.8219}\\
\hline
\bottomrule
\end{tabular} 
}
\end{table*}

==> Table/Complexity.tex <==
\begin{table}[!htb]
\centering
\huge 
\caption{Complexity Analysis on Matrix Completion Methods, $r_k$ (usually $r_k \geq r$) denotes an estimated rank at the $k$th iteration of SVD, $y$ denotes the number of subsets of $S$, $n_\text{p}$ denotes the number of search candidates, $n_\text{q}$ denotes the number of query items, $n=n_\text{p}+n_\text{q}$ denotes the total number of data samples, $T$ denotes the total number of iterations.}
\label{tab:Complexity} 
\resizebox{1\columnwidth}{!}{  
\begin{tabular}{lll}
\toprule
\hline
\textbf{Methods}        & \textbf{Computation Complexity} & \textbf{Storage Complexity} \\ \hline 
\textbf{BPMF}\cite{mnih2007probabilistic} & $O((n^2r^2 + nr^3)T)$  & $O(2nr + \|\Omega \|_0)$    \\
\textbf{FGSR}\cite{fan2019factor}        & $O((n^2r)T)$           & $O(2nr + \|\Omega \|_0)$    \\ \hline
\textbf{CMC}\cite{li2020scalable}        & $O((n^3/y^2)T)$        & $O(n^2 + \|\Omega \|_0)$    \\
\textbf{DMC}\cite{li2015estimating}       & $O((n^3)T)$            & $O(n^2 + \|\Omega \|_0)$    \\
\textbf{SMC}\cite{ma2024fast}       & $O(n_\text{p}^3+(n^2+\log n)T)$            & $O(n^2 + \|\Omega \|_0)$    \\ \hline
\textbf{NNFN}\cite{wang2021scalable}     & $O((n^2r_k)T)$         & $O(n^2 + \|\Omega \|_0)$        \\
\textbf{facNNFN}\cite{wang2021scalable}   & $O((n^2r+nr^2)T)$      & $O(2nr + \|\Omega\|_0)$     \\ \hline
\textbf{SMCNN (OURS)}  & $O((n^2r)T)$           & $O(nr + \|\Omega \|_0)$      \\
\textbf{SMCNmF (OURS) } & $O((n^2r+nr^2)T) $     & $O(nr + \|\Omega \|_0)$      \\ \hline
\bottomrule
\end{tabular}
}
\end{table}
 

==> Table/RMSE/s4q2.tex <==
 \begin{table}[!htb]
\centering
\scriptsize
\caption{Comparisons of RMSE, Recall@top20\%, nDCG@top20\% with $m=4,000$ search candidates and $n=200$ query items, where missing ratio $\rho =\{0.7,0.8,0.9\}$, rank $r = 100$, $\lambda = 0.001$, $\gamma = 0.001$, and $T = 10,000$. The top 2 performances are highlighted in bold.} 
\label{tab:rmse:s4q2}  
\resizebox{0.9\columnwidth}{!}{  
\begin{tabular}{cc|c|ccc|ccc|ccc}
\toprule
\hline
\multicolumn{3}{c|}{\multirow{2}{*}{\textbf{Dataset/Method}}}                      & \multicolumn{3}{c|}{\textbf{0.7}}                    & \multicolumn{3}{c|}{\textbf{0.8}}                    & \multicolumn{3}{c}{\textbf{0.9}}                \\ \cline{4-12}
\multicolumn{3}{c|}{}                                                                                         & \textbf{RMSE}   & \textbf{Recall} & \textbf{nDCG}   & \textbf{RMSE}   & \textbf{Recall} & \textbf{nDCG}   & \multicolumn{1}{c}{\textbf{RMSE}} & \multicolumn{1}{c}{\textbf{Recall}} & \multicolumn{1}{c}{\textbf{nDCG}} \\ \hline
\multicolumn{1}{c|}{\multirow{12}{*}{\textbf{GoogleNews}}} & \multirow{4}{*}{\textbf{MVI}} & \textbf{MEAN}\cite{kim2004reuse}   & 3.3690          & 0.5688          & 0.7410          & 2.2554          & 0.6576          & 0.7690          & 2.1283          & 0.5655          & 0.7841          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{LR}\cite{seber2012linear}     & 1.7977          & 0.5860          & 0.7675          & 2.5076          & 0.6787          & 0.7940          & 1.2371          & 0.5690          & 0.7985          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{GR}\cite{balzano2010online}     & 2.4633          & 0.5666          & 0.7814          & 2.3733          & 0.6268          & 0.7645          & 3.2717          & 0.5708          & 0.7982          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{KFMC}\cite{fan2019online}   & 1.2486          & 0.5620          & 0.7986          & 1.1440          & 0.6829          & 0.7506          & 1.7434          & 0.5703          & 0.7732          \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{2}{*}{\textbf{MF}}  & \textbf{FGSR}\cite{fan2019factor}   & 1.4100          & 0.5741          & 0.7890          & 1.2310          & 0.6723          & 0.7780          & 1.4140          & 0.5704          & 0.7542          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{BPMF}\cite{mnih2007probabilistic}   & 1.5140          & 0.5856          & 0.7835          & 1.2100          & 0.6752          & 0.7410          & 1.6530          & 0.5713          & 0.7240          \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{3}{*}{\textbf{PSD}} & \textbf{CMC}\cite{li2015estimating}    & 0.7718          & 0.6202          & 0.7841          & 0.6944          & 0.5680          & 0.7560          & 0.6667          & 0.5739          & 0.7340          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{DMC}\cite{li2020scalable}    & 0.7823          & 0.6262          & 0.7853          & 0.7131          & 0.5680          & 0.7533          & 0.6551          & 0.5717          & 0.7230          \\ 
\multicolumn{1}{c|}{}                                     &                               &  \textbf{FMC}\cite{ma2024fast}    & 0.7491                     & 0.6398                     & 0.7565                     & 0.6731                     & 0.6576                     & 0.7488                     & 0.5999 & 0.6157 & 0.7910 \\  \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{2}{*}{\textbf{LoR}}  & \textbf{NNFN}\cite{wang2021scalable}    & 0.8441          & 0.6196          & 0.7154          & 0.7190          & 0.5622          & 0.7636          & 0.8662          & 0.6534          & 0.7531          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{facNNFN}\cite{wang2021scalable} & 0.8760          & 0.6202          & 0.7129          & 1.2210          & 0.6202          & 0.7532          & 0.8949          & 0.6202          & 0.7514          \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{2}{*}{\textbf{OUR}} & \textbf{SMCNN}    & \textbf{0.7233} & \textbf{0.6438} & \textbf{0.7749} & \textbf{0.6543} & \textbf{0.6708} & \textbf{0.7966} & \textbf{0.5970} & \textbf{0.6398} & \textbf{0.8242} \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{SMCNmF}   & \textbf{0.7134} & \textbf{0.6438} & \textbf{0.7749} & \textbf{0.6534} & \textbf{0.6708} & \textbf{0.7966} & \textbf{0.5979} & \textbf{0.6408} & \textbf{0.8082} \\ \hline
\multicolumn{1}{c|}{\multirow{12}{*}{\textbf{ImageNet}}}  & \multirow{4}{*}{\textbf{MVI}} & \textbf{MEAN}\cite{kim2004reuse}   & 3.9934          & 0.5114          & 0.6779          & 3.2631          & 0.4982          & 0.6792          & 3.3933          & 0.6948          & 0.6990          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{LR}\cite{seber2012linear}     & 4.1411          & 0.4958          & 0.6731          & 2.3855          & 0.4791          & 0.6784          & 2.1861          & 0.6780          & 0.6970          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{GR}\cite{balzano2010online}     & 2.9941          & 0.5081          & 0.6798          & 1.3837          & 0.4789          & 0.6787          & 2.1985          & 0.6776          & 0.6780          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{KFMC}\cite{fan2019online}   & 3.8410          & 0.4928          & 0.6712          & 1.3476          & 0.4595          & 0.6784          & 2.1902          & 0.6773          & 0.6873          \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{2}{*}{\textbf{MF}}  & \textbf{FGSR}\cite{fan2019factor}   & 1.4130          & 0.5623          & 0.6701          & 1.2130          & 0.5139          & 0.6813          & 1.5310          & 0.7130          & 0.7123          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{BPMF}\cite{mnih2007probabilistic}   & 1.1441          & 0.5675          & 0.6710          & 1.1410          & 0.5621          & 0.6841          & 1.6350          & 0.6527          & 0.7412          \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{3}{*}{\textbf{PSD}} & \textbf{CMC}\cite{li2015estimating}    & 0.6915          & 0.5715          & 0.6713          & 0.7270          & 0.5610          & 0.6834          & 0.6494          & 0.6148          & \textbf{0.7416} \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{DMC}\cite{li2020scalable}    & 0.6906          & 0.5752          & 0.6709          & 0.7249          & 0.5749          & 0.6865          & 0.6017          & 0.6312          & 0.7683          \\ 
\multicolumn{1}{c|}{}                                     &                               &  \textbf{FMC}\cite{ma2024fast}    & 0.6559                     & 0.6278                     & 0.6965                     & 0.6509                     & 0.6005                     & 0.6540                     & 0.5943 & 0.7193 & 0.7200 \\  \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{2}{*}{\textbf{LoR}}  & \textbf{NNFN}\cite{wang2021scalable}    & 1.0752          & 0.5762          & 0.7012          & 0.6532          & 0.5616          & 0.6875          & 0.9279          & 0.6480          & 0.7682          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{facNNFN}\cite{wang2021scalable} & 1.0920          & 0.5765          & 0.7083          & 0.7534          & 0.5980          & 0.6884          & 1.4600          & 0.6595          & 0.7684          \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{2}{*}{\textbf{OUR}} & \textbf{SMCNN}    & \textbf{0.6105} & \textbf{0.6323} & \textbf{0.7177} & \textbf{0.5983} & \textbf{0.6000} & \textbf{0.6956} & \textbf{0.5634} & \textbf{0.7036} & \textbf{0.7929} \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{SMCNmF}   & \textbf{0.6063} & \textbf{0.6296} & \textbf{0.7047} & \textbf{0.5967} & \textbf{0.6042} & \textbf{0.6956} & \textbf{0.5730} & \textbf{0.7080} & \textbf{0.7443} \\ \hline
\multicolumn{1}{c|}{\multirow{12}{*}{\textbf{MNIST}}}     & \multirow{4}{*}{\textbf{MVI}} & \textbf{MEAN}\cite{kim2004reuse}   & 2.3830          & 0.6334          & 0.7395          & 2.2710          & 0.5817          & 0.6434          & 2.1403          & 0.6006          & 0.7719          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{LR}\cite{seber2012linear}     & 1.7297          & 0.6978          & 0.7399          & 2.4529          & 0.5784          & 0.6513          & 2.2151          & 0.6179          & 0.8090          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{GR}\cite{balzano2010online}     & 1.4909          & 0.6894          & 0.7693          & 1.3451          & 0.5796          & 0.6591          & 2.2178          & 0.6140          & 0.8238          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{KFMC}\cite{fan2019online}   & 1.4100          & 0.6870          & 0.7692          & 0.9418          & 0.5783          & 0.7591          & 3.3177          & 0.6130          & 0.8431          \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{2}{*}{\textbf{MF}}  & \textbf{FGSR}\cite{fan2019factor}   & 1.4210          & 0.6712          & 0.7813          & 1.1320          & 0.5740          & 0.7140          & 1.4100          & 0.6340          & 0.8510          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{BPMF}\cite{mnih2007probabilistic}   & 1.6500          & 0.6792          & 0.7817          & 1.2130          & 0.5741          & 0.7340          & 1.5344          & 0.5653          & 0.8410          \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{3}{*}{\textbf{PSD}} & \textbf{CMC}\cite{li2015estimating}    & 0.8563          & 0.6725          & 0.7820          & 0.8680          & 0.6278          & 0.7642          & 0.6510          & 0.6068          & 0.8134          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{DMC}\cite{li2020scalable}    & 0.8012          & 0.6735          & 0.7636          & 0.7162          & 0.6195          & 0.7410          & 0.6718          & 0.6130          & 0.8510          \\ 
\multicolumn{1}{c|}{}                                     &                               &  \textbf{FMC}\cite{ma2024fast}  & 0.7627                     & 0.7274                     & 0.7965                     & 0.7316                     & 0.6774                     & 0.6997                     & 0.6506 & 0.6289 & 0.8920 \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{2}{*}{\textbf{LoR}}  & \textbf{NNFN}\cite{wang2021scalable}    & 0.8210          & 0.6700          & 0.7895          & 0.8221          & 0.6338          & 0.7389          & 0.7506          & 0.6060          & 0.8410          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{facNNFN}\cite{wang2021scalable} & 1.2712          & 0.6378          & 0.8124          & 3.9790          & 0.6085          & 0.7843          & 1.0840          & 0.6097          & 0.8410          \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{2}{*}{\textbf{OUR}} & \textbf{SMCNN}    & \textbf{0.7843} & \textbf{0.7363} & \textbf{0.8193} & \textbf{0.6260} & \textbf{0.6460} & \textbf{0.7844} & \textbf{0.6425} & \textbf{0.6533} & \textbf{0.8948} \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{SMCNmF}   & \textbf{0.7328} & \textbf{0.7288} & \textbf{0.8033} & \textbf{0.6518} & \textbf{0.6708} & \textbf{0.7869} & \textbf{0.6415} & \textbf{0.6500} & \textbf{0.8931} \\ \hline
\multicolumn{1}{c|}{\multirow{12}{*}{\textbf{PROTEIN}}}   & \multirow{4}{*}{\textbf{MVI}} & \textbf{MEAN}\cite{kim2004reuse}   & 2.2905          & 0.5811          & 0.6594          & 2.1765          & 0.5906          & 0.6841          & 2.0652          & 0.6760          & 0.7395          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{LR}\cite{seber2012linear}     & 2.6848          & 0.5739          & 0.6157          & 1.4045          & 0.6362          & 0.6483          & 3.1311          & 0.6741          & 0.7289          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{GR}\cite{balzano2010online}     & 1.6753          & 0.6801          & 0.6940          & 1.5771          & 0.5526          & 0.7894          & 2.2553          & 0.6721          & 0.7385          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{KFMC}\cite{fan2019online}   & 1.0109          & 0.6060          & 0.7140          & 1.8972          & 0.5381          & 0.7642          & 1.5423          & 0.6726          & 0.7232          \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{2}{*}{\textbf{MF}}  & \textbf{FGSR}\cite{fan2019factor}   & 1.1800          & 0.6097          & 0.7214          & 1.1710          & 0.5969          & 0.7684          & 1.1380          & 0.6969          & 0.7421          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{BPMF}\cite{mnih2007probabilistic}   & 0.7658          & 0.6069          & 0.7431          & 0.3799          & 0.5969          & 0.7542          & 1.1082          & 0.6969          & 0.7582          \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{3}{*}{\textbf{PSD}} & \textbf{CMC}\cite{li2015estimating}    & 0.8477          & 0.6931          & 0.7814          & 0.7888          & 0.6062          & 0.7851          & 0.6585          & 0.6887          & 0.8234          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{DMC}\cite{li2020scalable}    & 0.8308          & 0.6931          & 0.7843          & 0.7807          & 0.6130          & 0.7522          & 0.6497          & 0.6886          & 0.8334          \\ 
\multicolumn{1}{c|}{}                                     &                               &  \textbf{FMC}\cite{ma2024fast}    & 0.7559                     & 0.7054                     & 0.7942                     & 0.6565                     & 0.6181                     & 0.7988                     & 0.6249 & 0.7009 & 0.7819 \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{2}{*}{\textbf{LoR}}  & \textbf{NNFN}\cite{wang2021scalable}    & 0.8532          & 0.6831          & 0.7843          & 0.8209          & 0.6234          & 0.7600          & 0.6529          & 0.6801          & 0.8459          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{facNNFN}\cite{wang2021scalable} & 1.2420          & 0.7105          & 0.7854          & 1.3930          & 0.6070          & 0.7673          & 1.9589          & 0.7116          & 0.8415          \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{2}{*}{\textbf{OUR}} & \textbf{SMCNN}    & \textbf{0.7506} & \textbf{0.7183} & \textbf{0.7917} & \textbf{0.6574} & \textbf{0.6313} & \textbf{0.7934} & \textbf{0.5390} & \textbf{0.7323} & \textbf{0.8477} \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{SMCNmF}   & \textbf{0.7526} & \textbf{0.7198} & \textbf{0.7913} & \textbf{0.6446} & \textbf{0.6333} & \textbf{0.7914} & \textbf{0.5828} & \textbf{0.7080} & \textbf{0.8413} \\ \hline
\multicolumn{1}{c|}{\multirow{12}{*}{\textbf{CIFAR10}}}     & \multirow{4}{*}{\textbf{MVI}} & \textbf{MEAN}\cite{kim2004reuse}   & 3.3780          & 0.6833          & 0.5710          & 2.2661          & 0.5178          & 0.6772          & 2.1414          & 0.6795          & 0.7840          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{LR}\cite{seber2012linear}     & 1.8263          & 0.6746          & 0.5909          & 1.5263          & 0.5777          & 0.6774          & 2.2605          & 0.6704          & 0.7640          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{GR}\cite{balzano2010online}     & 2.4690          & 0.6233          & 0.5900          & 2.3683          & 0.5800          & 0.6814          & 1.2526          & 0.6070          & 0.7840          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{KFMC}\cite{fan2019online}   & 1.1935          & 0.6798          & 0.5890          & 1.0112          & 0.5774          & 0.6802          & 1.6271          & 0.6075          & 0.7410          \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{2}{*}{\textbf{MF}}  & \textbf{BPMF}\cite{mnih2007probabilistic}   & 1.1230          & 0.6812          & 0.6013          & 1.3100          & 0.6131          & 0.6813          & 1.5130          & 0.6210          & 0.7568          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{FGSR}\cite{fan2019factor}   & 1.0213          & 0.6712          & 0.6140          & 1.4100          & 0.6234          & 0.6801          & 1.6252          & 0.6723          & 0.7853          \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{3}{*}{\textbf{PSD}} & \textbf{CMC}\cite{li2015estimating}    & 0.7939          & 0.7113          & 0.7140          & 0.7648          & 0.6728          & 0.6831          & 0.7136          & 0.6803          & 0.7825          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{DMC}\cite{li2020scalable}    & 0.7931          & 0.7135          & 0.7520          & 0.7628          & 0.6715          & 0.6841          & 0.7292          & 0.6800          & 0.7409          \\ \multicolumn{1}{c|}{}                                     &                               &  \textbf{FMC}\cite{ma2024fast}    &  0.7573  & 0.7114  &  0.7944  & 0.7664 &0.6715  &  0.7883 & 0.6711 & 0.7083 & 0.7997 \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{2}{*}{\textbf{LoR}}  & \textbf{NNFN}\cite{wang2021scalable}    & 0.7940          & 0.6704          & 0.7851          & 0.7304          & 0.6753          & 0.6823          & 0.8056          & 0.6819          & 0.7714          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{facNNFN}\cite{wang2021scalable} & 1.0913          & 0.6701          & 0.8140          & 3.4564          & 0.6705          & 0.6864          & 1.0032          & 0.6230          & 0.8014          \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{2}{*}{\textbf{OUR}} & \textbf{SMCNN}    & \textbf{0.7527} & \textbf{0.7234} & \textbf{0.8947} & \textbf{0.7189} & \textbf{0.6318} & \textbf{0.7942} & \textbf{0.6486} & \textbf{0.7204} & \textbf{0.8310} \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{SMCNmF}   & \textbf{0.7506} & \textbf{0.7146} & \textbf{0.8948} & \textbf{0.7179} & \textbf{0.6295} & \textbf{0.7795} & \textbf{0.6493} & \textbf{0.7267} & \textbf{0.8310}\\
\hline
\bottomrule
\end{tabular} 
}
\end{table}

==> Table/RMSE/s5q2.tex <==
 \begin{table}[!htb]
\centering
\scriptsize
\caption{Comparisons of RMSE, Recall@top20\%, nDCG@top20\% with $m=5,000$ search candidates and $n=200$ query items, where missing ratio $\rho =\{0.7,0.8,0.9\}$, rank $r = 100$, $\lambda = 0.001$, $\gamma = 0.001$, and $T = 10,000$. The top 2 performances are highlighted in bold.} 
\label{tab:rmse:s5q2}  
\resizebox{0.9\columnwidth}{!}{ 
\begin{tabular}{cc|c|ccc|ccc|ccc}
\toprule
\hline
\multicolumn{3}{c|}{\multirow{2}{*}{\textbf{Dataset/Method}}}                      & \multicolumn{3}{c|}{\textbf{0.7}}                    & \multicolumn{3}{c|}{\textbf{0.8}}                    & \multicolumn{3}{c}{\textbf{0.9}}                \\ \cline{4-12}
\multicolumn{3}{c|}{}                                                                                         & \textbf{RMSE}   & \textbf{Recall} & \textbf{nDCG}   & \textbf{RMSE}   & \textbf{Recall} & \textbf{nDCG}   & \multicolumn{1}{c}{\textbf{RMSE}} & \multicolumn{1}{c}{\textbf{Recall}} & \multicolumn{1}{c}{\textbf{nDCG}} \\ \hline
\multicolumn{1}{c|}{\multirow{12}{*}{\textbf{GoogleNews}}} & \multirow{4}{*}{\textbf{MVI}} & \textbf{MEAN}\cite{kim2004reuse}   & 1.2584          & 0.5858          & 0.6831          & 10.1389         & 0.6540          & 0.7659          & 7.6430          & 0.5234          & 0.7920          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{LR}\cite{seber2012linear}     & 8.4157          & 0.4404          & 0.7452          & 10.2086         & 0.6456          & 0.7303          & 10.1178         & 0.6140          & 0.7841          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{GR}\cite{balzano2010online}     & 8.4923          & 0.4509          & 0.7543          & 8.3270          & 0.6456          & 0.7243          & 2.3420          & 0.5610          & 0.8123          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{KFMC}\cite{fan2019online}   & 7.3655          & 0.4551          & 0.7680          & 7.2029          & 0.6433          & 0.7334          & 10.1501         & 0.5923          & 0.8101          \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{2}{*}{\textbf{MF}}  & \textbf{FGSR}\cite{fan2019factor}   & 1.4112          & 0.6642          & 0.7654          & 3.1230          & 0.6746          & 0.7866          & 1.3210          & 0.6023          & 0.7415          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{BPMF}\cite{mnih2007probabilistic}   & 1.4310          & 0.6842          & 0.7965          & 2.1430          & 0.6902          & 0.7946          & 1.3410          & 0.6123          & 0.7187          \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{3}{*}{\textbf{PSD}} & \textbf{CMC}\cite{li2015estimating}    & 0.8996          & 0.7014          & 0.7134          & 0.8331          & 0.6817          & 0.8019          & 0.7165          & 0.5150          & 0.7040          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{DMC}\cite{li2020scalable}    & 0.8849          & 0.7155          & 0.7290          & 0.7187          & 0.6879          & 0.8342          & 0.7536          & 0.6151          & 0.7020          \\ 
\multicolumn{1}{c|}{}                                     &                               &  \textbf{FMC}\cite{ma2024fast}    &  0.7278                     & 0.7680                     & 0.7398                     & 0.6934                     & 0.6932                     & 0.7997                     & 0.7158 & 0.6185 & 0.7949 \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{2}{*}{\textbf{LoR}}  & \textbf{NNFN}\cite{wang2021scalable}    & 1.3555          & 0.6218          & 0.7262          & 0.7222          & 0.6851          & 0.8669          & 0.7528          & 0.6146          & 0.8164          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{facNNFN}\cite{wang2021scalable} & 1.2407          & 0.6657          & 0.7460          & 3.9181          & 0.6313          & 0.8080          & 3.1120          & 0.5933          & 0.7907          \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{2}{*}{\textbf{OUR}} & \textbf{SMCNN}    & \textbf{0.7278} & \textbf{0.7625} & \textbf{0.7493} & \textbf{0.6813} & \textbf{0.6980} & \textbf{0.8188} & \textbf{0.7031} & \textbf{0.6421} & \textbf{0.8172} \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{SMCNmF}   & \textbf{0.7241} & \textbf{0.7625} & \textbf{0.7314} & \textbf{0.6960} & \textbf{0.6988} & \textbf{0.8050} & \textbf{0.7041} & \textbf{0.6421} & \textbf{0.8219} \\ \hline
\multicolumn{1}{c|}{\multirow{12}{*}{\textbf{ImageNet}}}  & \multirow{4}{*}{\textbf{MVI}} & \textbf{MEAN}\cite{kim2004reuse}   & 10.2715         & 0.6856          & 0.7644          & 9.1607          & 0.5654          & 0.7641          & 10.0561         & 0.5950          & 0.8120          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{LR}\cite{seber2012linear}     & 10.5570         & 0.6711          & 0.7874          & 8.3064          & 0.5653          & 0.7052          & 8.0986          & 0.6214          & 0.8230          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{GR}\cite{balzano2010online}     & 9.4037          & 0.6770          & 0.7547          & 7.3779          & 0.5644          & 0.7402          & 8.3322          & 0.6151          & 0.8310          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{KFMC}\cite{fan2019online}   & 9.8087          & 0.6746          & 0.8450          & 6.6336          & 0.5675          & 0.7260          & 8.3866          & 0.6041          & 0.7980          \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{2}{*}{\textbf{MF}}  & \textbf{FGSR}\cite{fan2019factor}   & 2.4312          & 0.7130          & 0.8135          & 1.3210          & 0.5642          & 0.7821          & 2.3120          & 0.5980          & 0.7387          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{BPMF}\cite{mnih2007probabilistic}   & 2.5410          & 0.8123          & 0.8145          & 1.4200          & 0.5695          & 0.7823          & 2.4230          & 0.5902          & 0.7065          \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{3}{*}{\textbf{PSD}} & \textbf{CMC}\cite{li2015estimating}    & 0.7504          & 0.7347          & 0.8342          & 0.6355          & 0.5691          & 0.7841          & 0.5670          & 0.6317          & 0.6988 \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{DMC}\cite{li2020scalable}    & 0.7358          & 0.7335          & 0.9042          & 0.6375          & 0.5693          & 0.7854          & 0.5344          & 0.6331          & 0.7011          \\ 
\multicolumn{1}{c|}{}                                     &                               &  \textbf{FMC}\cite{ma2024fast}    & 0.7682                     & 0.7315                     & 0.8748                     & 0.6582                     & 0.6392                     & 0.7680                     & 0.5589 & 0.6780 & 0.6997 \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{2}{*}{\textbf{LoR}}  & \textbf{NNFN}\cite{wang2021scalable}    & 0.7311          & 0.7143          & 0.9004          & 0.7415          & 0.5685          & 0.7910          & 0.8016          & 0.6358          & 0.8878          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{facNNFN}\cite{wang2021scalable} & 3.9142          & 0.7033          & 0.8536          & 3.3542          & 0.5679          & 0.7841          & 3.1220          & 0.6350          & 0.8338          \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{2}{*}{\textbf{OUR}} & \textbf{SMCNN}    & \textbf{0.7110} & \textbf{0.7433} & \textbf{0.9070} & \textbf{0.6187} & \textbf{0.6446} & \textbf{0.7986} & \textbf{0.5128} & \textbf{0.6625} & \textbf{0.7896} \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{SMCNmF}   & \textbf{0.7104} & \textbf{0.7363} & \textbf{0.9065} & \textbf{0.6238} & \textbf{0.6429} & \textbf{0.7984} & \textbf{0.5127} & \textbf{0.6620} & \textbf{0.7897} \\ \hline
\multicolumn{1}{c|}{\multirow{12}{*}{\textbf{MNIST}}}     & \multirow{4}{*}{\textbf{MVI}} & \textbf{MEAN}\cite{kim2004reuse}   & 8.6230          & 0.7516          & 0.6987          & 8.2431          & 0.6551          & 0.8123          & 6.8579          & 0.5542          & 0.7964          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{LR}\cite{seber2012linear}     & 2.6224          & 0.6882          & 0.6996          & 2.1784          & 0.7867          & 0.8103          & 1.3979          & 0.5854          & 0.7993          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{GR}\cite{balzano2010online}     & 2.5311          & 0.6838          & 0.6994          & 2.3440          & 0.7933          & 0.7918          & 1.8814          & 0.5748          & 0.7860          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{KFMC}\cite{fan2019online}   & 1.9770          & 0.6890          & 0.6997          & 2.0105          & 0.8524          & 0.8013          & 1.8398          & 0.5801          & 0.7912          \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{2}{*}{\textbf{MF}}  & \textbf{FGSR}\cite{fan2019factor}   & 1.4321          & 0.7142          & 0.7131          & 0.9310          & 0.7814          & 0.8452          & 1.2310          & 0.6131          & 0.8012          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{BPMF}\cite{mnih2007probabilistic}   & 1.5430          & 0.8432          & 0.8123          & 0.9341          & 0.7913          & 0.8452          & 1.4310          & 0.7013          & 0.8123          \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{3}{*}{\textbf{PSD}} & \textbf{CMC}\cite{li2015estimating}    & 0.8326          & 0.8410          & 0.8451          & 0.6575          & 0.8170          & 0.7854          & 0.5769          & 0.7548          & 0.8431          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{DMC}\cite{li2020scalable}    & 0.7634          & 0.8424          & 0.8544          & 0.6705          & 0.8198          & 0.7859          & 0.5954          & 0.7408          & 0.8534          \\ 
\multicolumn{1}{c|}{}                                     &                               &  \textbf{FMC}\cite{ma2024fast}    &  0.7358                     & 0.8306                     & 0.8974                     & 0.6355                     & 0.7919                     & 0.8268                     & 0.5623 & 0.7278 & 0.7997 \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{2}{*}{\textbf{LoR}}  & \textbf{NNFN}\cite{wang2021scalable}    & 1.0968          & 0.5883          & 0.8654          & 0.8194          & 0.5880          & 0.7899          & 0.7688          & 0.5550          & 0.8134          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{facNNFN}\cite{wang2021scalable} & 39.9580         & 0.2163          & 0.8943          & 17.7280         & 0.2163          & 0.7899          & 4.2018          & 0.2163          & 0.8313          \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{2}{*}{\textbf{OUR}} & \textbf{SMCNN}    & \textbf{0.7197} & \textbf{0.8688} & \textbf{0.8969} & \textbf{0.6237} & \textbf{0.8021} & \textbf{0.8370} & \textbf{0.5653} & \textbf{0.7696} & \textbf{0.8580} \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{SMCNmF}   & \textbf{0.7128} & \textbf{0.8563} & \textbf{0.8973} & \textbf{0.6233} & \textbf{0.8208} & \textbf{0.8364} & \textbf{0.5438} & \textbf{0.7460} & \textbf{0.8640} \\ \hline
\multicolumn{1}{c|}{\multirow{12}{*}{\textbf{PROTEIN}}}   & \multirow{4}{*}{\textbf{MVI}} & \textbf{MEAN}\cite{kim2004reuse}   & 10.2665         & 0.4787          & 0.7908          & 10.1544         & 0.5650          & 0.7665          & 10.0504         & 0.4523          & 0.7340          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{LR}\cite{seber2012linear}     & 10.4684         & 0.4319          & 0.8397          & 8.2502          & 0.5600          & 0.7237          & 8.0753          & 0.5940          & 0.7234          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{GR}\cite{balzano2010online}     & 9.4332          & 0.4656          & 0.8282          & 5.3721          & 0.6430          & 0.7353          & 8.2056          & 0.5420          & 0.7134          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{KFMC}\cite{fan2019online}   & 8.4820          & 0.4749          & 0.8268          & 6.3198          & 0.5643          & 0.7252          & 7.5452          & 0.6144          & 0.7412          \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{2}{*}{\textbf{MF}}  & \textbf{FGSR}\cite{fan2019factor}   & 1.3214          & 0.5431          & 0.8256          & 2.1310          & 0.5960          & 0.7843          & 5.3400          & 0.6120          & 0.7431          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{BPMF}\cite{mnih2007probabilistic}   & 1.4325          & 0.5640          & 0.8265          & 1.4100          & 0.5489          & 0.8121          & 4.1340          & 0.6120          & 0.7176          \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{3}{*}{\textbf{PSD}} & \textbf{CMC}\cite{li2015estimating}    & 0.7314          & 0.6575          & 0.8445          & 0.6974          & 0.6414          & 0.8320          & 0.7783          & 0.6153          & 0.7031          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{DMC}\cite{li2020scalable}    & 0.7351          & 0.6582          & 0.8650          & 0.6794          & 0.6351          & 0.7913          & 0.7653          & 0.6148          & 0.6994          \\ 
\multicolumn{1}{c|}{}                                     &                               &  \textbf{FMC}\cite{ma2024fast}    & 0.6865                     & 0.6701                     & 0.7997                     & 0.6200                     & 0.6116                     & 0.7971                     & 0.6145 & 0.6475 & 0.7703 \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{2}{*}{\textbf{LoR}}  & \textbf{NNFN}\cite{wang2021scalable}    & 1.3492          & 0.5447          & 0.8308          & 0.6573          & 0.6413          & 0.8880          & 0.7810          & 0.6198          & 0.8619          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{facNNFN}\cite{wang2021scalable} & 7.2052          & 0.5001          & 0.8397          & 1.7311          & 0.5208          & 0.8247          & 1.8390          & 0.2203          & 0.8124          \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{2}{*}{\textbf{OUR}} & \textbf{SMCNN}    & \textbf{0.6508} & \textbf{0.6896} & \textbf{0.8755} & \textbf{0.6240} & \textbf{0.6104} & \textbf{0.8699} & \textbf{0.5735} & \textbf{0.6688} & \textbf{0.8858} \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{SMCNmF}   & \textbf{0.6442} & \textbf{0.6904} & \textbf{0.8663} & \textbf{0.6402} & \textbf{0.6167} & \textbf{0.8566} & \textbf{0.5900} & \textbf{0.6521} & \textbf{0.8838} \\ \hline
\multicolumn{1}{c|}{\multirow{12}{*}{\textbf{CIFAR10}}}     & \multirow{4}{*}{\textbf{MVI}} & \textbf{MEAN}\cite{kim2004reuse}   & 7.4454          & 0.5153          & 0.7839          & 4.8767          & 0.4820          & 0.6980          & 2.9687          & 0.6022          & 0.4976          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{LR}\cite{seber2012linear}     & 19.7330         & 0.3790          & 0.4998          & 9.8335          & 0.4834          & 0.6973          & 2.7372          & 0.5820          & 0.4961          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{GR}\cite{balzano2010online}     & 5.7612          & 0.5368          & 0.7576          & 3.4935          & 0.5072          & 0.6819          & 2.6397          & 0.5929          & 0.4777          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{KFMC}\cite{fan2019online}   & 2.1644          & 0.5655          & 0.7452          & 1.6547          & 0.4515          & 0.6102          & 1.4308          & 0.4112          & 0.4847          \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{2}{*}{\textbf{MF}}  & \textbf{BPMF}\cite{mnih2007probabilistic}   & 0.9310          & 0.5695          & 0.7650          & 1.0310          & 0.4450          & 0.6340          & 1.2120          & 0.5430          & 0.5440          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{FGSR}\cite{fan2019factor}   & 1.3100          & 0.5765          & 0.7065          & 1.4310          & 0.5530          & 0.6500          & 1.5340          & 0.6534          & 0.6432          \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{3}{*}{\textbf{PSD}} & \textbf{CMC}\cite{li2015estimating}    & 0.8773          & 0.5810          & 0.7855          & 0.8373          & 0.6192          & 0.6530          & 0.6735          & 0.5612          & 0.6735          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{DMC}\cite{li2020scalable}    & 0.8256          & 0.5802          & 0.7835          & 0.8121          & 0.6263          & 0.6530          & 0.5822          & 0.5672          & 0.6784          \\ 
\multicolumn{1}{c|}{}                                     &                               &  \textbf{FMC}\cite{ma2024fast}    &   0.6977 &  0.6486 &  0.7997  &  0.5975  &  0.6621  &  0.6972 & 0.5448 & 0.6028 & 0.7970 \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{2}{*}{\textbf{LoR}}  & \textbf{NNFN}\cite{wang2021scalable}    & 0.8202          & 0.5828          & 0.7864          & 0.7578          & 0.6015          & 0.6450          & 0.5797          & 0.5551          & 0.7812          \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{facNNFN}\cite{wang2021scalable} & 0.9890          & 0.6241          & 0.7847          & 1.6120          & 0.5417          & 0.6680          & 1.0512          & 0.6423          & 0.7832          \\ \cline{2-12}
\multicolumn{1}{c|}{}                                     & \multirow{2}{*}{\textbf{OUR}} & \textbf{SMCNN}    & \textbf{0.6868} & \textbf{0.6446} & \textbf{0.8555} & \textbf{0.5942} & \textbf{0.6960} & \textbf{0.6934} & \textbf{0.5213} & \textbf{0.6563} & \textbf{0.7975} \\
\multicolumn{1}{c|}{}                                     &                               & \textbf{SMCNmF}   & \textbf{0.6379} & \textbf{0.6429} & \textbf{0.8387} & \textbf{0.5841} & \textbf{0.6938} & \textbf{0.6941} & \textbf{0.5289} & \textbf{0.6583} & \textbf{0.7972}\\
\hline
\bottomrule
\end{tabular} 
}
\end{table}

==> Table/Rank/Ranktol.tex <==
\begin{table}[!htb]
\centering
\scriptsize
\caption{Rank($\hat{S}$), with $m=1,000$ search candidates and $n=200$ query items, where Rank($V$)=$r$=$100$ with various $\rho$, fixed $\lambda=0.001$, $\gamma =0.001$, and iterations $T=10,000$. Va1-Va5 denotes SMC\_F, SMC\_NR, }
\label{tab:Rank:Ranktol} 
\resizebox{1\columnwidth}{!}{    
% \scalebox{0.99}{
\begin{tabular}{c|c|ccccccccc}
\toprule
\hline
%\multicolumn{1}{l|}{\textbf{Datasets}} &\textbf{$\rho$}& \textbf{NNFN} & \textbf{facNNFN} & \textbf{SMCNN} & \textbf{SMCNmF} & \textbf{SMCNN\_F} & \textbf{SMCNN\_NR} & \textbf{SMC\_QN} & \textbf{SMCNN\_QN} & \textbf{SMCNmF\_QN} \\ \hline
\multicolumn{1}{l|}{\textbf{Datasets}} &\textbf{$\rho$}& \textbf{NNFN} & \textbf{facNNFN} & \textbf{SMCNN} & \textbf{SMCNmF} & \textbf{Va1} & \textbf{Va2} & \textbf{Va3} & \textbf{Va4} & \textbf{Va5} \\ \hline
\multirow{5}{*}{\textbf{ImageNet}} & \textbf{0.5}    & 172    & 151   & 69  & 72   & 69 & 72 & 72    & 66 & 66  \\
  & \textbf{0.6}    & 169    & 148   & 69  & 72   & 72 & 75 & 69    & 72 & 75  \\
  & \textbf{0.7}    & 175    & 175   & 75  & 78   & 72 & 78 & 72    & 72 & 75  \\
  & \textbf{0.8}    & 178    & 166   & 93  & 93   & 93 & 90 & 87    & 87 & 87  \\
  & \textbf{0.9}    & 187    & 187   & 105 & 102  & 102    & 99 & 99    & 102 & 102 \\ \hline
\multirow{5}{*}{\textbf{MNIST}}    & \textbf{0.5}    & 120    & 142   & 30  & 30   & 30 & 30 & 30    & 30 & 30  \\
  & \textbf{0.6}    & 111    & 157   & 30  & 30   & 30 & 30 & 30    & 30 & 30  \\
  & \textbf{0.7}    & 102    & 172   & 30  & 30   & 30 & 30 & 30    & 30 & 30  \\
  & \textbf{0.8}    & 99 & 90    & 30  & 33   & 30 & 30 & 30    & 30 & 30  \\
  & \textbf{0.9}    & 102    & 93    & 69  & 69   & 69 & 72 & 72    & 72 & 72  \\ \hline
\multirow{5}{*}{\textbf{PROTEIN}}  & \textbf{0.5}    & 163    & 148   & 78  & 75   & 78 & 75 & 75    & 78 & 78  \\
  & \textbf{0.6}    & 163    & 148   & 75  & 75   & 78 & 72 & 75    & 78 & 78  \\
  & \textbf{0.7}    & 169    & 148   & 75  & 81   & 81 & 81 & 75    & 75 & 75  \\
  & \textbf{0.8}    & 172    & 148   & 90  & 93   & 90 & 93 & 81    & 81 & 75  \\
  & \textbf{0.9}    & 172    & 160   & 102 & 105  & 102    & 102 & 102   & 99 & 102 \\ \hline
\multirow{5}{*}{\textbf{CIFAR}}    & \textbf{0.5}    & 196    & 163   & 30  & 30   & 33 & 30 & 30    & 30 & 33  \\
  & \textbf{0.6}    & 96 & 74    & 30  & 33   & 33 & 33 & 30    & 33 & 30  \\
  & \textbf{0.7}    & 90 & 90    & 30  & 30   & 33 & 33 & 33    & 33 & 33  \\
  & \textbf{0.8}    & 90 & 94    & 39  & 42   & 39 & 42 & 42    & 42 & 42  \\
  & \textbf{0.9}    & 114    & 98    & 90  & 87   & 90 & 87 & 90    & 87 & 87  \\ \hline
\multirow{5}{*}{\textbf{GoogleNews}} & \textbf{0.5} &  122 & 111 &  72    & 75 & 75  &74  &75  &75  &75    \\
 & \textbf{0.6} & 151   &124 & 73  &  76 & 78   & 75 & 75  & 73 &75   \\
 & \textbf{0.7} &  176&  148 &  73   &  83 &  85 &  83  &85 & 85   &85    \\
 & \textbf{0.8} &  197   & 153 &  87 &  94 &  93 &  92  &93 & 93   &93    \\
 & \textbf{0.9} &  195&  162 & 102&  103 & 103 &104 &103 &103 &105  \\
\hline
  \bottomrule
\end{tabular} 
}
\end{table}

==> Table/Rank/hatSRank.tex <==
\begin{table}[!htb]
\centering
\huge
\caption{Rank of factorized submatrix $V$, Rank($\hat{V}$), on various datasets, with $m=1,000$ search candidates and $n=200$ query items, where missing ratio $\rho=\{0.7,0.8,0.9\}$, rank of $V$ is $r$=$100$, $\lambda=0.001$, $\gamma =0.001$, and $T=10,000$. Va1-Va5 denotes SMC\_F, SMC\_NR, SMC\_QN, SMCNN\_QN, SMCNmF\_QN.}
\label{tab:Rank:hatV} 
\resizebox{\columnwidth}{!}{ 
\begin{tabular}{c|c|cccccccccc}
\toprule
\hline
\textbf{Datasets}                    & $\rho$       & \textbf{facNNFN} & \textbf{FGSR} & \textbf{BPMF} & \textbf{Va1} & \textbf{Va2} & \textbf{Va3} & \textbf{Va4} & \textbf{Va5} & \textbf{SMCNN} & \textbf{SMCNmF} \\ \hline
\multirow{3}{*}{\textbf{ImageNet}}   & \textbf{0.7} & 109              & 113           & 100           & 130             & 102              & 81               & 84                 & 81                  & 80            & 80             \\
                                     & \textbf{0.8} & 110              & 114           & 100           & 142             & 102              & 86               & 84                 & 82                  & 82            & 81             \\
                                     & \textbf{0.9} & 112              & 114           & 100           & 141             & 101              & 95               & 85                 & 92                  & 91            & 91             \\ \hline
\multirow{3}{*}{\textbf{MNIST}}      & \textbf{0.7} & 126              & 121           & 100           & 111             & 112              & 85               & 92                 & 90                  & 83            & 93             \\
                                     & \textbf{0.8} & 126              & 128           & 100           & 111             & 102              & 87               & 92                 & 89                  & 83            & 93             \\
                                     & \textbf{0.9} & 126              & 131           & 100           & 111             & 103              & 88               & 94                 & 94                  & 84            & 83             \\  \hline
\multirow{3}{*}{\textbf{PROTEIN}}    & \textbf{0.7} & 129              & 131           & 100           & 111             & 104              & 86               & 89                 & 86                  & 89            & 87             \\
                                     & \textbf{0.8} & 129              & 128           & 100           & 121             & 102              & 85               & 92                 & 89                  & 89            & 89             \\
                                     & \textbf{0.9} & 132              & 130           & 100           & 118             & 104              & 89               & 95                 & 95                  & 91            & 93             \\  \hline
\multirow{3}{*}{\textbf{CIFAR}}      & \textbf{0.7} & 117              & 118           & 100           & 111             & 104              & 87               & 90                 & 86                  & 84            & 84             \\
                                     & \textbf{0.8} & 127              & 120           & 100           & 111             & 104              & 89               & 89                 & 87                  & 83            & 83             \\
                                     & \textbf{0.9} & 128              & 124           & 100           & 113             & 104              & 93               & 95                 & 93                  & 89            & 88             \\  \hline
\multirow{3}{*}{\textbf{GoogleNews}} & \textbf{0.7} & 106              & 112           & 100           & 106             & 102              & 89               & 90                 & 88                  & 90            & 91             \\
                                     & \textbf{0.8} & 116              & 110           & 100           & 106             & 107              & 94               & 89                 & 90                  & 92            & 91             \\
                                     & \textbf{0.9} & 116              & 110           & 100           & 111             & 108              & 97               & 95                 & 94                  & 93            & 94            \\
                                     \hline
                                     \bottomrule
\end{tabular}
}
\end{table}

==> Table/Time/TimeAll.tex <==
\begin{table}[!htb]
\centering 
\caption{Comparisons of Running Time (seconds) with $m=1,000$ search candidates and $n=200$ query items with different stopping criteria, where missing ratio $\rho =\{0.7,0.8,0.9\}$.  }
\label{tab:timetol} 
\resizebox{0.6\columnwidth}{!}{  
\begin{tabular}{l|l|lll|lll}
\toprule
\hline 
\multicolumn{1}{l|}{\multirow{2}{*}{\textbf{Datasets}}} & \multicolumn{1}{l|}{\multirow{2}{*}{\textbf{Methods}}} & \multicolumn{3}{c|}{$tol$=1e-4}                                     & \multicolumn{3}{c}{$T$=10,000}                  \\ \cline{3-8}
\multicolumn{1}{l|}{}                          & \multicolumn{1}{l|}{}                         & \multicolumn{1}{c}{\textbf{0.7}} & \multicolumn{1}{c}{\textbf{0.8}} & \multicolumn{1}{c|}{\textbf{0.9}} & \multicolumn{1}{c}{\textbf{0.7}} & \multicolumn{1}{c}{\textbf{0.8}} & \multicolumn{1}{c}{\textbf{0.9}} \\ \hline


\multirow{3}{*}{\textbf{GoogleNews}}   & \textbf{CMC}\cite{li2020scalable} & 90.480                           & 133.680                          & 113.360                          & 933.440                          & 953.984                          & 910.324                          \\
                                   & \textbf{DMC}\cite{li2015estimating} & 164.200                          & 164.583                          & 160.834                          & 986.925                          & 951.092                          & 863.088                          \\
                                   & \textbf{SMC}\cite{ma2024fast} & 174.598                          & 188.044                          & 161.380                          & 1004.345                         & 983.393                          & 950.984                          \\ \hline
\multirow{3}{*}{\textbf{ImageNet}} & \textbf{CMC}\cite{li2020scalable} & 142.000                          & 201.321                          & 202.604                          & 647.364                          & 845.126                          & 882.515                          \\
                                   & \textbf{DMC}\cite{li2015estimating} & 302.083                          & 302.083                          & 302.083                          & 899.752                          & 854.716                          & 944.558                          \\
                                   & \textbf{SMC}\cite{ma2024fast} & 339.370                          & 324.144                          & 210.620                          & 918.410                          & 881.343                          & 959.742                          \\ \hline
\multirow{3}{*}{\textbf{MNIST}}    & \textbf{CMC}\cite{li2020scalable} & 165.320                          & 154.250                          & 165.320                          & 929.354                          & 884.899                          & 811.374                          \\
                                   & \textbf{DMC}\cite{li2015estimating} & 305.430                          & 301.042                          & 302.604                          & 991.231                          & 901.923                          & 836.731                          \\ 
                                   & \textbf{SMC}\cite{ma2024fast} & 236.387                          & 285.015                          & 291.890                          & 950.964                          & 956.076                          & 811.294                          \\ \hline
\multirow{3}{*}{\textbf{PROTEIN}}  & \textbf{CMC}\cite{li2020scalable} & 90.480                           & 133.680                          & 113.360                          & 958.414                          & 830.618                          & 811.103                          \\
                                   & \textbf{DMC}\cite{li2015estimating} & 164.200                          & 164.583                          & 160.834                          & 945.510                          & 838.923                          & 824.212                          \\
                                   & \textbf{SMC}\cite{ma2024fast} & 158.420                          & 166.458                          & 150.901                          & 971.378                          & 891.337                          & 856.123                          \\ \hline
\multirow{3}{*}{\textbf{CIFAR10}}    & \textbf{CMC}\cite{li2020scalable} & 90.480                           & 133.680                          & 113.360                          & 918.800                          & 807.828                          & 856.735                          \\
                                   & \textbf{DMC}\cite{li2015estimating} & 164.200                          & 164.583                          & 160.834                          & 979.401                          & 811.595                          & 822.524                          \\
                                   & \textbf{SMC}\cite{ma2024fast} & 164.189                          & 173.216                          & 181.758                          & 1007.641                         & 807.416                          & 831.172               \\
                                   \hline
                                   \bottomrule
\end{tabular} 
}
\end{table}
